When No-Rejection Learning is Consistent for Regression with Rejection

Learning with rejection has been a prototypical model for studying the human-AI interaction on prediction tasks. Upon the arrival of a sample instance, the model first uses a rejector to decide whether to accept and use the AI predictor to make a prediction or reject and defer the sample to humans. Learning such a model changes the structure of the original loss function and often results in undesirable non-convexity and inconsistency issues. For the classification with rejection problem, several works develop consistent surrogate losses for the joint learning of the predictor and the rejector, while there have been fewer works for the regression counterpart. This paper studies the regression with rejection (RwR) problem and investigates a no-rejection learning strategy that uses all the data to learn the predictor. We first establish the consistency for such a strategy under the weak realizability condition. Then for the case without the weak realizability, we show that the excessive risk can also be upper bounded with the sum of two parts: prediction error and calibration error. Lastly, we demonstrate the advantage of such a proposed learning strategy with empirical evidence.

==> Rebuttal/informs2014.tex <==
%%
%% This is file `ormsv080.bst',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `ay,nat,nm-revv1,jnrlst,dt-beg,yr-per,yrp-per,note-yr,thtit-a,vol-bf,volp-blk,pp-last,num-xser,numser,ser-vol,ser-ed,jnm-x,bkpg-x,pre-edn,doi,in-x,ppx,ed,abr,ednx,mth-bare,ord,jabr,xand,url,url-blk,em-it,plntx,')
%% ----------------------------------------
%% *** ormsv080 050112 ***
%% 
%% Copyright 1994-2004 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2004/02/09 4.13 (PWD, AO, DPC)]
 %   For use with BibTeX version 0.99a or later
 %-------------------------------------------------------------------
 % This bibliography style file is intended for texts in ENGLISH
 % This is an author-year citation style bibliography. As such, it is
 % non-standard LaTeX, and requires a special package file to function properly.
 % Such a package is    natbib.sty   by Patrick W. Daly
 % The form of the \bibitem entries is
 %   \bibitem[Jones et al.(1990)]{key}...
 %   \bibitem[Jones et al.(1990)Jones, Baker, and Smith]{key}...
 % The essential feature is that the label (the part in brackets) consists
 % of the author names, as they should appear in the citation, with the year
 % in parentheses following. There must be no space before the opening
 % parenthesis!
 % With natbib v5.3, a full list of authors may also follow the year.
 % In natbib.sty, it is possible to define the type of enclosures that is
 % really wanted (brackets or parentheses), but in either case, there must
 % be parentheses in the label.
 % The \cite command functions as follows:
 %   \citet{key} ==>>                Jones et al. (1990)
 %   \citet*{key} ==>>               Jones, Baker, and Smith (1990)
 %   \citep{key} ==>>                (Jones et al., 1990)
 %   \citep*{key} ==>>               (Jones, Baker, and Smith, 1990)
 %   \citep[chap. 2]{key} ==>>       (Jones et al., 1990, chap. 2)
 %   \citep[e.g.][]{key} ==>>        (e.g. Jones et al., 1990)
 %   \citep[e.g.][p. 32]{key} ==>>   (e.g. Jones et al., p. 32)
 %   \citeauthor{key} ==>>           Jones et al.
 %   \citeauthor*{key} ==>>          Jones, Baker, and Smith
 %   \citeyear{key} ==>>             1990
 %---------------------------------------------------------------------

ENTRY
  { address
    author
    booktitle
    chapter
    doi
    edition
    editor
    eid
    howpublished
    institution
    journal
    key
    month
    note
    number
    organization
    pages
    publisher
    school
    series
    title
    type
    url
    volume
    year
  }
  {}
  { label extra.label sort.label short.list }
INTEGERS { output.state before.all mid.sentence after.sentence after.block }
FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}
STRINGS { s t}
FUNCTION {output.nonnull}
{ 's :=
  output.state mid.sentence =
    { ", " * write$ }
    { output.state after.block =
        { add.period$ write$
          newline$
          "\newblock " write$
        }
        { output.state before.all =
            'write$
            { add.period$ " " * write$ }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}
FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}
FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}
FUNCTION {fin.entry}
{ add.period$
  write$
  newline$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}
FUNCTION {new.sentence}
{ output.state after.block =
    'skip$
    { output.state before.all =
        'skip$
        { after.sentence 'output.state := }
      if$
    }
  if$
}
FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}

FUNCTION {date.block}
{
  new.block
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}
FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}
FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}
STRINGS {z}
FUNCTION {remove.dots}
{ 'z :=
  ""
  { z empty$ not }
  { z #1 #1 substring$
    z #2 global.max$ substring$ 'z :=
    duplicate$ "." = 'pop$
      { * }
    if$
  }
  while$
}
FUNCTION {new.block.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.block
  if$
}
FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}
FUNCTION {emphasize}
{ duplicate$ empty$
    { pop$ "" }
    { "{\it " swap$ * "\/}" * }
  if$
}
FUNCTION {bolden}
{ duplicate$ empty$
    { pop$ "" }
    { "{\bf " swap$ * "}" * }
  if$
}
FUNCTION {tie.or.space.prefix}
{ duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$
}

FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }
 % Here are the language-specific definitions for explicit words.
 % Each function has a name bbl.xxx where xxx is the English word.
 % The language selected here is ENGLISH
FUNCTION {bbl.and}
{ "and"}

FUNCTION {bbl.etal}
{ "et~al." }

FUNCTION {bbl.editors}
{ "eds." }

FUNCTION {bbl.editor}
{ "ed." }

FUNCTION {bbl.edby}
{ "edited by" }

FUNCTION {bbl.edition}
{ "ed." }

FUNCTION {bbl.volume}
{ "vol." }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "no." }

FUNCTION {bbl.nr}
{ "no." }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "" }

FUNCTION {bbl.page}
{ "" }

FUNCTION {bbl.chapter}
{ "chap." }

FUNCTION {bbl.techrep}
{ "Tech. Rep." }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "Ph.D. thesis" }

FUNCTION {bbl.first}
{ "1st" }

FUNCTION {bbl.second}
{ "2nd" }

FUNCTION {bbl.third}
{ "3rd" }

FUNCTION {bbl.fourth}
{ "4th" }

FUNCTION {bbl.fifth}
{ "5th" }

FUNCTION {bbl.st}
{ "st" }

FUNCTION {bbl.nd}
{ "nd" }

FUNCTION {bbl.rd}
{ "rd" }

FUNCTION {bbl.th}
{ "th" }

MACRO {jan} {"Jan."}

MACRO {feb} {"Feb."}

MACRO {mar} {"Mar."}

MACRO {apr} {"Apr."}

MACRO {may} {"May"}

MACRO {jun} {"Jun."}

MACRO {jul} {"Jul."}

MACRO {aug} {"Aug."}

MACRO {sep} {"Sep."}

MACRO {oct} {"Oct."}

MACRO {nov} {"Nov."}

MACRO {dec} {"Dec."}

FUNCTION {eng.ord}
{ duplicate$ "1" swap$ *
  #-2 #1 substring$ "1" =
     { bbl.th * }
     { duplicate$ #-1 #1 substring$
       duplicate$ "1" =
         { pop$ bbl.st * }
         { duplicate$ "2" =
             { pop$ bbl.nd * }
             { "3" =
                 { bbl.rd * }
                 { bbl.th * }
               if$
             }
           if$
          }
       if$
     }
   if$
}

MACRO {acmcs} {"ACM Comput. Surv."}

MACRO {acta} {"Acta Inf."}

MACRO {cacm} {"Commun. ACM"}

MACRO {ibmjrd} {"IBM J. Res. Dev."}

MACRO {ibmsj} {"IBM Syst.~J."}

MACRO {ieeese} {"IEEE Trans. Software Eng."}

MACRO {ieeetc} {"IEEE Trans. Comput."}

MACRO {ieeetcad}
 {"IEEE Trans. Comput. Aid. Des."}

MACRO {ipl} {"Inf. Process. Lett."}

MACRO {jacm} {"J.~ACM"}

MACRO {jcss} {"J.~Comput. Syst. Sci."}

MACRO {scp} {"Sci. Comput. Program."}

MACRO {sicomp} {"SIAM J. Comput."}

MACRO {tocs} {"ACM Trans. Comput. Syst."}

MACRO {tods} {"ACM Trans. Database Syst."}

MACRO {tog} {"ACM Trans. Graphic."}

MACRO {toms} {"ACM Trans. Math. Software"}

MACRO {toois} {"ACM Trans. Office Inf. Syst."}

MACRO {toplas} {"ACM Trans. Progr. Lang. Syst."}

MACRO {tcs} {"Theor. Comput. Sci."}

FUNCTION {bibinfo.check}
{ swap$
  duplicate$ missing$
    {
      pop$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ pop$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
FUNCTION {bibinfo.warn}
{ swap$
  duplicate$ missing$
    {
      swap$ "missing " swap$ * " in " * cite$ * warning$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ "empty " swap$ * " in " * cite$ * warning$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
FUNCTION {format.url}
{ url empty$
    { "" }
    { "\urlprefix\url{" url * "}" * }
  if$
}

STRINGS  { bibinfo}
INTEGERS { nameptr namesleft numnames }

FUNCTION {format.names}
{ 'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      duplicate$ #1 >
        { "{ff~}{vv~}{ll}{, jj}" }
        { "{vv~}{ll}{, ff}{, jj}" }
      if$
      format.name$
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              "," *
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {
                  " " * bbl.etal *
                }
                { " " * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  } if$
}
FUNCTION {format.names.ed}
{
  'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{ff~}{vv~}{ll}{, jj}"
      format.name$
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              "," *
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {

                  " " * bbl.etal *
                }
                { " " * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  } if$
}
FUNCTION {format.key}
{ empty$
    { key field.or.null }
    { "" }
  if$
}

FUNCTION {format.authors}
{ author "author" format.names
}
FUNCTION {get.bbl.editor}
{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }

FUNCTION {format.editors}
{ editor "editor" format.names duplicate$ empty$ 'skip$
    {
      "," *
      " " *
      get.bbl.editor
      *
    }
  if$
}
FUNCTION {format.doi}
{ doi "doi" bibinfo.check
  duplicate$ empty$ 'skip$
    {
      new.block
      "\doi{" swap$ * "}" *
    }
  if$
}
FUNCTION {format.note}
{
 note empty$
    { "" }
    { note #1 #1 substring$
      duplicate$ "{" =
        'skip$
        { output.state mid.sentence =
          { "l" }
          { "u" }
        if$
        change.case$
        }
      if$
      note #2 global.max$ substring$ * "note" bibinfo.check
    }
  if$
}

FUNCTION {format.title}
{ title
  duplicate$ empty$ 'skip$
    { "t" change.case$ }
  if$
  "title" bibinfo.check
}
FUNCTION {format.full.names}
{'s :=
 "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv~}{ll}" format.name$
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {
                  " " * bbl.etal *
                }
                {
                  numnames #2 >
                    { "," * }
                    'skip$
                  if$
                  bbl.and
                  space.word * t *
                }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {author.editor.key.full}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { editor format.full.names }
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {author.key.full}
{ author empty$
    { key empty$
         { cite$ #1 #3 substring$ }
          'key
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {editor.key.full}
{ editor empty$
    { key empty$
         { cite$ #1 #3 substring$ }
          'key
      if$
    }
    { editor format.full.names }
  if$
}

FUNCTION {make.full.names}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.key.full
    { type$ "proceedings" =
        'editor.key.full
        'author.key.full
      if$
    }
  if$
}

FUNCTION {output.bibitem}
{ newline$
  "\bibitem[{" write$
  label write$
  ")" make.full.names duplicate$ short.list =
     { pop$ }
     { * }
   if$
  "}]{" * write$
  cite$ write$
  "}" write$
  newline$
  ""
  before.all 'output.state :=
}

FUNCTION {n.dashify}
{
  't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
        { t #1 #2 substring$ "--" = not
            { "--" *
              t #2 global.max$ substring$ 't :=
            }
            {   { t #1 #1 substring$ "-" = }
                { "-" *
                  t #2 global.max$ substring$ 't :=
                }
              while$
            }
          if$
        }
        { t #1 #1 substring$ *
          t #2 global.max$ substring$ 't :=
        }
      if$
    }
  while$
}

FUNCTION {word.in}
{ "" }

FUNCTION {format.date}
{ year "year" bibinfo.check duplicate$ empty$
    {
      "empty year in " cite$ * "; set to ????" * warning$
       pop$ "????"
    }
    'skip$
  if$
  extra.label *
  before.all 'output.state :=
  after.sentence 'output.state :=
}
FUNCTION {format.btitle}
{ title "title" bibinfo.check
  duplicate$ empty$ 'skip$
    {
      emphasize
    }
  if$
}
FUNCTION {either.or.check}
{ empty$
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}
FUNCTION {format.bvolume}
{ volume empty$
    { "" }
    { bbl.volume volume tie.or.space.prefix
      "volume" bibinfo.check * *
      series "series" bibinfo.check
      duplicate$ empty$ 'pop$
        { emphasize ", " * swap$ * }
      if$
      "volume and number" number either.or.check
    }
  if$
}
FUNCTION {format.number.series}
{ volume empty$
    { number empty$
        { series field.or.null }
        { series empty$
            { number "number" bibinfo.check }
            { output.state mid.sentence =
                { bbl.number }
                { bbl.number capitalize }
              if$
              number tie.or.space.prefix "number" bibinfo.check * *
              bbl.in space.word *
              series "series" bibinfo.check *
            }
          if$
        }
      if$
    }
    { "" }
  if$
}
FUNCTION {is.num}
{ chr.to.int$
  duplicate$ "0" chr.to.int$ < not
  swap$ "9" chr.to.int$ > not and
}

FUNCTION {extract.num}
{ duplicate$ 't :=
  "" 's :=
  { t empty$ not }
  { t #1 #1 substring$
    t #2 global.max$ substring$ 't :=
    duplicate$ is.num
      { s swap$ * 's := }
      { pop$ "" 't := }
    if$
  }
  while$
  s empty$
    'skip$
    { pop$ s }
  if$
}

FUNCTION {convert.edition}
{ extract.num "l" change.case$ 's :=
  s "first" = s "1" = or
    { bbl.first 't := }
    { s "second" = s "2" = or
        { bbl.second 't := }
        { s "third" = s "3" = or
            { bbl.third 't := }
            { s "fourth" = s "4" = or
                { bbl.fourth 't := }
                { s "fifth" = s "5" = or
                    { bbl.fifth 't := }
                    { s #1 #1 substring$ is.num
                        { s eng.ord 't := }
                        { edition 't := }
                      if$
                    }
                  if$
                }
              if$
            }
          if$
        }
      if$
    }
  if$
  t
}

FUNCTION {format.edition}
{ edition duplicate$ empty$ 'skip$
    {
      convert.edition
      output.state mid.sentence =
        { "l" }
        { "t" }
      if$ change.case$
      "edition" bibinfo.check
      " " * bbl.edition *
    }
  if$
}
INTEGERS { multiresult }
FUNCTION {multi.page.check}
{ 't :=
  #0 'multiresult :=
    { multiresult not
      t empty$ not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
        { #1 'multiresult := }
        { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}
FUNCTION {format.pages}
{ pages duplicate$ empty$ 'skip$
    { duplicate$ multi.page.check
        {
          n.dashify
        }
        {
        }
      if$
      "pages" bibinfo.check
    }
  if$
}
FUNCTION {format.journal.pages}
{ pages duplicate$ empty$ 'pop$
    { swap$ duplicate$ empty$
        { pop$ pop$ format.pages }
        {
          " " *
          swap$
          n.dashify
          "pages" bibinfo.check
          *
        }
      if$
    }
  if$
}
FUNCTION {format.journal.eid}
{ eid "eid" bibinfo.check
  duplicate$ empty$ 'pop$
    { swap$ duplicate$ empty$ 'skip$
      {
          " " *
      }
      if$
      swap$ *
    }
  if$
}
FUNCTION {format.vol.num.pages}
{ volume field.or.null
  duplicate$ empty$ 'skip$
    {
      "volume" bibinfo.check
    }
  if$
  bolden
  number "number" bibinfo.check duplicate$ empty$ 'skip$
    {
      swap$ duplicate$ empty$
        { "there's a number but no volume in " cite$ * warning$ }
        'skip$
      if$
      swap$
      "(" swap$ * ")" *
    }
  if$ *
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    { "" }
    { type empty$
        { bbl.chapter }
        { type "l" change.case$
          "type" bibinfo.check
        }
      if$
      chapter tie.or.space.prefix
      "chapter" bibinfo.check
      * *
    }
  if$
}

FUNCTION {format.booktitle}
{
  booktitle "booktitle" bibinfo.check
  emphasize
}
FUNCTION {format.in.ed.booktitle}
{ format.booktitle duplicate$ empty$ 'skip$
    {
      format.bvolume duplicate$ empty$ 'pop$
        { ", " swap$ * * }
      if$
      editor "editor" format.names.ed duplicate$ empty$ 'pop$
        {
          "," *
          " " *
          get.bbl.editor
          ", " *
          * swap$
          * }
      if$
      word.in swap$ *
    }
  if$
}
FUNCTION {format.thesis.type}
{ type duplicate$ empty$
    'pop$
    { swap$ pop$
      "t" change.case$ "type" bibinfo.check
    }
  if$
}
FUNCTION {format.tr.number}
{ number "number" bibinfo.check
  type duplicate$ empty$
    { pop$ bbl.techrep }
    'skip$
  if$
  "type" bibinfo.check
  swap$ duplicate$ empty$
    { pop$ "t" change.case$ }
    { tie.or.space.prefix * * }
  if$
}
FUNCTION {format.article.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}
FUNCTION {format.book.crossref}
{ volume duplicate$ empty$
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      pop$ word.in
    }
    { bbl.volume
      capitalize
      swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *
    }
  if$
  " \cite{" * crossref * "}" *
}
FUNCTION {format.incoll.inproc.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}
FUNCTION {format.org.or.pub}
{ 't :=
  ""
  address empty$ t empty$ and
    'skip$
    {
      t empty$
        { address "address" bibinfo.check *
        }
        { t *
          address empty$
            'skip$
            { ", " * address "address" bibinfo.check * }
          if$
        }
      if$
    }
  if$
}
FUNCTION {format.publisher.address}
{ publisher "publisher" bibinfo.warn format.org.or.pub
}

FUNCTION {format.organization.address}
{ organization "organization" bibinfo.check format.org.or.pub
}

FUNCTION {article}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.block
  crossref missing$
    {
      journal
      "journal" bibinfo.check
      emphasize
      "journal" output.check
      add.blank
      format.vol.num.pages output
    }
    { format.article.crossref output.nonnull
    }
  if$
  eid empty$
    { format.journal.pages }
    { format.journal.eid }
  if$
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}
FUNCTION {book}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      editor format.key output
    }
    { format.authors output.nonnull
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      new.block
      format.edition output
      new.sentence
      format.number.series output
      format.publisher.address output
    }
    {
      new.block
      format.book.crossref output.nonnull
    }
  if$
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}
FUNCTION {booklet}
{ output.bibitem
  format.authors output
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.block
  howpublished "howpublished" bibinfo.check output
  address "address" bibinfo.check output
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}

FUNCTION {inbook}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      editor format.key output
    }
    { format.authors output.nonnull
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  crossref missing$
    {
      format.bvolume output
      format.chapter.pages "chapter and pages" output.check
      new.block
      format.edition output
      new.sentence
      format.number.series output
      format.publisher.address output
    }
    {
      format.chapter.pages "chapter and pages" output.check
      new.block
      format.book.crossref output.nonnull
    }
  if$
  format.pages "pages" output.check
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}

FUNCTION {incollection}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.edition output
      format.chapter.pages output
      new.sentence
      format.number.series output
      format.publisher.address output
    }
    { format.incoll.inproc.crossref output.nonnull
      format.chapter.pages output
    }
  if$
  format.pages "pages" output.check
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}
FUNCTION {inproceedings}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      new.sentence
      format.number.series output
      publisher empty$
        { format.organization.address output }
        { organization "organization" bibinfo.check output
          format.publisher.address output
        }
      if$
    }
    { format.incoll.inproc.crossref output.nonnull
    }
  if$
  format.pages "pages" output.check
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}
FUNCTION {conference} { inproceedings }
FUNCTION {manual}
{ output.bibitem
  format.authors output
  author format.key output
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  organization address new.block.checkb
  organization "organization" bibinfo.check output
  address "address" bibinfo.check output
  format.edition output
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}

FUNCTION {mastersthesis}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title
  "title" output.check
  new.block
  bbl.mthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}

FUNCTION {misc}
{ output.bibitem
  format.authors output
  author format.key output
  format.date "year" output.check
  date.block
  format.title output
  new.block
  howpublished "howpublished" bibinfo.check output
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}
FUNCTION {phdthesis}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title
  "title" output.check
  new.block
  bbl.phdthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
  format.editors output
  editor format.key output
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  format.bvolume output
  new.sentence
  format.number.series output
  publisher empty$
    { format.organization.address output }
    { organization "organization" bibinfo.check output
      format.publisher.address output
    }
  if$
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}

FUNCTION {techreport}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title
  "title" output.check
  new.block
  format.tr.number output.nonnull
  institution "institution" bibinfo.warn output
  address "address" bibinfo.check output
  format.doi output
  new.block
  format.url output
  new.block
  format.note output
  fin.entry
}

FUNCTION {unpublished}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  format.doi output
  new.block
  format.url output
  new.block
  format.note "note" output.check
  fin.entry
}

FUNCTION {default.type} { misc }
READ
FUNCTION {sortify}
{ purify$
  "l" change.case$
}
INTEGERS { len }
FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}
FUNCTION {format.lab.names}
{ 's :=
  "" 't :=
  s #1 "{vv~}{ll}" format.name$
  s num.names$ duplicate$
  #2 >
    { pop$
      " " * bbl.etal *
    }
    { #2 <
        'skip$
        { s #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            {
              " " * bbl.etal *
            }
            { bbl.and space.word * s #2 "{vv~}{ll}" format.name$
              * }
          if$
        }
      if$
    }
  if$
}

FUNCTION {author.key.label}
{ author empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {author.editor.key.label}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { editor format.lab.names }
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {editor.key.label}
{ editor empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { editor format.lab.names }
  if$
}

FUNCTION {calc.short.authors}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.key.label
    { type$ "proceedings" =
        'editor.key.label
        'author.key.label
      if$
    }
  if$
  'short.list :=
}

FUNCTION {calc.label}
{ calc.short.authors
  short.list
  "("
  *
  year duplicate$ empty$
     { pop$ "????" }
     'skip$
  if$
  *
  'label :=
}

FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv{ } }{ll{ }}{  ff{ }}{  jj{ }}"
      format.name$ 't :=
      nameptr #1 >
        {
          "   "  *
          namesleft #1 = t "others" = and
            { "zzzzz" * }
            { t sortify * }
          if$
        }
        { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}
FUNCTION {author.sort}
{ author empty$
    { key empty$
        { "to sort, need author or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
        { key empty$
            { "to sort, need author, editor, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {editor.sort}
{ editor empty$
    { key empty$
        { "to sort, need editor or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { editor sort.format.names }
  if$
}
FUNCTION {presort}
{ calc.label
  label sortify
  "    "
  *
  type$ "book" =
  type$ "inbook" =
  or
    'author.editor.sort
    { type$ "proceedings" =
        'editor.sort
        'author.sort
      if$
    }
  if$
  #1 entry.max$ substring$
  'sort.label :=
  sort.label
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {presort}
SORT
STRINGS { last.label next.extra }
INTEGERS { last.extra.num number.label }
FUNCTION {initialize.extra.label.stuff}
{ #0 int.to.chr$ 'last.label :=
  "" 'next.extra :=
  #0 'last.extra.num :=
  #0 'number.label :=
}
FUNCTION {forward.pass}
{ last.label label =
    { last.extra.num #1 + 'last.extra.num :=
      last.extra.num int.to.chr$ 'extra.label :=
    }
    { "a" chr.to.int$ 'last.extra.num :=
      "" 'extra.label :=
      label 'last.label :=
    }
  if$
  number.label #1 + 'number.label :=
}
FUNCTION {reverse.pass}
{ next.extra "b" =
    { "a" 'extra.label := }
    'skip$
  if$
  extra.label 'next.extra :=
  extra.label
  duplicate$ empty$
    'skip$
    { "{\natexlab{" swap$ * "}}" * }
  if$
  'extra.label :=
  label extra.label * 'label :=
}
EXECUTE {initialize.extra.label.stuff}
ITERATE {forward.pass}
REVERSE {reverse.pass}
FUNCTION {bib.sort.order}
{ sort.label
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}
ITERATE {bib.sort.order}
SORT
FUNCTION {begin.bib}
{ preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{" number.label int.to.str$ * "}" *
  write$ newline$
  "\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi"
  write$ newline$
  "\expandafter\ifx\csname url\endcsname\relax"
  write$ newline$
  "  \def\url#1{{\tt #1}}\fi"
  write$ newline$
  "\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi"
  write$ newline$
  "\expandafter\ifx\csname urlstyle\endcsname\relax"
  write$ newline$
  "  \expandafter\ifx\csname doi\endcsname\relax"
  write$ newline$
  "  \def\doi#1{doi:\discretionary{}{}{}#1}\fi \else"
  write$ newline$
  "  \expandafter\ifx\csname doi\endcsname\relax"
  write$ newline$
  "  \def\doi{doi:\discretionary{}{}{}\begingroup \urlstyle{rm}\Url}\fi \fi"
  write$ newline$
}
EXECUTE {begin.bib}
EXECUTE {init.state.consts}
ITERATE {call.type$}
FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}
EXECUTE {end.bib}
%% End of customized bst file
%%
%% End of file `ormsv080.bst'.


==> Rebuttal/informs3.tex <==
%% Updated to handle e-companions (EC) (see corresponding templates)
%% 12/04/2007 fixed error in \quote
%% 11/11/2010 added template disclaimer in \theARTICLETOP
%% 12/20/2010 reworked type sizes ("per popular demand"); \OneAndAHalfSizedXI - default
%% 02/23/2012 Fixed typo in "@otatefalse" (s/b "@rotatefalse")
%% 08/09/2012 Fixed typo in a message "mansucript" (s/b "manuscript")
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesClass{informs3}
  [2012/08/09 v0.95
   LaTeX document class for articles submitted to INFORMS]

\RequirePackage{amsmath,amssymb,ifthen,url,graphicx,color,array,theorem}

%%%=============================================================================
%%% A simplified reloading scheme for Computer Modern fonts
%% Variation of `ot1cmr.fd',
\DeclareFontFamily{OT1}{cmr}{\hyphenchar\font45 }
\DeclareFontShape{OT1}{cmr}{m}{n}{<-10>gen*cmr<10->cmr10}{}
\DeclareFontShape{OT1}{cmr}{m}{sl}{<->cmti10}{} % slanted type discouraged
\DeclareFontShape{OT1}{cmr}{m}{it}{<5><6><7>cmti7<8>cmti8<9>cmti9<10->cmti10}{}
\DeclareFontShape{OT1}{cmr}{m}{sc}{<5->cmcsc10}{}
\DeclareFontShape{OT1}{cmr}{m}{ui}{<->cmu10}{}
%%%%%%%% bold extended series
\DeclareFontShape{OT1}{cmr}{bx}{n}{<5><6><7><8><9>gen*cmbx<10->cmbx10}{}
\DeclareFontShape{OT1}{cmr}{bx}{sl}{<->cmbxti10}{}  % slanted type discouraged
\DeclareFontShape{OT1}{cmr}{bx}{it}{<->cmbxti10}{}
\DeclareFontShape{OT1}{cmr}{bx}{ui}{<->ssub*cmr/m/ui}{}
\DeclareFontShape{OT1}{cmtt}{m}{n}{<5><6><7><8>cmtt8<9>cmtt9<10->cmtt10}{}
%%%%%% make sure subst shapes are available
\DeclareFontShape{OT1}{cmtt}{m}{it}{<->cmitt10}{}
\DeclareFontShape{OT1}{cmtt}{m}{sl}{<->cmitt10}{} % slanted type discouraged
\DeclareFontShape{OT1}{cmtt}{m}{sc}{<->cmtcsc10}{}
\DeclareFontShape{OT1}{cmtt}{m}{ui}{<->ssub*cmtt/m/it}{}
\DeclareFontShape{OT1}{cmtt}{bx}{n}{<->ssub*cmtt/m/n}{}
\DeclareFontShape{OT1}{cmtt}{bx}{it}{<->ssub*cmtt/m/it}{}
\DeclareFontShape{OT1}{cmtt}{bx}{ui}{<->ssub*cmtt/m/it}{}
\DeclareFontShape{OT1}{cmss}{m}{n}{<->cmss10}{}
% Font undefined, therefore substituted
\DeclareFontShape{OT1}{cmss}{m}{it}{<->cmssi10}{}
\DeclareFontShape{OT1}{cmss}{m}{sl}{<->cmssi10}{}
%%%%%%% Font/shape undefined, therefore substituted
\DeclareFontShape{OT1}{cmss}{m}{sc}{<->sub*cmr/m/sc}{}
%%%%%%% Font/shape undefined, therefore substituted
\DeclareFontShape{OT1}{cmss}{m}{ui}{<->sub*cmr/m/ui}{}
%%%%%%%% semibold condensed series
\DeclareFontShape{OT1}{cmss}{sbc}{n}{<->cmssdc10}{}
%%%%%%%%% bold extended series
\DeclareFontShape{OT1}{cmss}{bx}{n}{<->cmssbx10}{}
%%%%%%% Font/shape undefined, therefore substituted
\DeclareFontShape{OT1}{cmss}{bx}{ui}{<->sub*cmr/bx/ui}{}
\DeclareFontShape{OML}{cmm}{m}{it}{<5><6><7><8><9>gen*cmmi<10->cmmi10}{}
\DeclareFontShape{OML}{cmm}{b}{it}{<5><6><7><8><9>gen*cmmib<10->cmmib10}{}
\DeclareFontShape{OML}{cmm}{bx}{it}{<->ssub*cmm/b/it}{}
%%%%%%%%%%%%%%%%%%-AMS-msam+msbm fonts
\DeclareFontFamily{U}{msa}{}
\DeclareFontShape{U}{msa}{m}{n}{<-> msam10}{}
\DeclareFontFamily{U}{msb}{}
\DeclareFontShape{U}{msb}{m}{n}{<-> msbm10}{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareOldFontCommand{\RMrm}{\rmfamily\mdseries\upshape}{\mathrm}
\DeclareOldFontCommand{\RMit}{\rmfamily\mdseries\itshape}{\mathit}
\DeclareOldFontCommand{\RMbf}{\rmfamily\bfseries\upshape}{\mathbf}
\DeclareOldFontCommand{\RMbi}{\rmfamily\bfseries\itshape}{\mathbi}
%
\def\thit{\it}% Theorem italic does not exist in CM
%
\DeclareOldFontCommand{\RMsf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\RMsfi}{\normalfont\sffamily\itshape}{\mathsfi}
\DeclareOldFontCommand{\RMtt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\RMsc}{\normalfont\scshape}{\@nomath\sc}
%
\def\ROMAN{%
\let\rm=\RMrm
\let\it=\RMit
\let\bf=\RMbf
\let\bi=\RMbi
\let\sf=\RMsf
\let\sfi=\RMsfi
\let\tt=\RMtt
\let\sc=\RMsc
}
\ROMAN % default
\DeclareOldFontCommand{\SFrm}{\sffamily\mdseries\upshape}{\mathrm}
\DeclareOldFontCommand{\SFit}{\sffamily\mdseries\itshape}{\mathit}
\DeclareOldFontCommand{\SFbf}{\sffamily\bfseries\upshape}{\mathbf}
%
\def\SANS{%
  \let\rm=\SFrm
  \let\it=\SFit
  \let\bf=\SFbf
  \sffamily\mdseries\upshape\selectfont
}
\def\cal#1{\mathcal{#1}}% CMM
%
%************************-b-bold math letters
%%% Adding bold symbols
\DeclareSymbolFont{boperators}   {OT1}{cmr} {bx}{n}
\DeclareSymbolFont{bletters}     {OML}{cmm} {b}{it}
\DeclareSymbolFont{bsymbols}     {OMS}{cmsy}{b}{n}
%
\DeclareMathSymbol{\BFa}{\mathalpha}{boperators}{`a}
\DeclareMathSymbol{\BFb}{\mathalpha}{boperators}{`b}
\DeclareMathSymbol{\BFc}{\mathalpha}{boperators}{`c}
\DeclareMathSymbol{\BFd}{\mathalpha}{boperators}{`d}
\DeclareMathSymbol{\BFe}{\mathalpha}{boperators}{`e}
\DeclareMathSymbol{\BFf}{\mathalpha}{boperators}{`f}
\DeclareMathSymbol{\BFg}{\mathalpha}{boperators}{`g}
\DeclareMathSymbol{\BFh}{\mathalpha}{boperators}{`h}
\DeclareMathSymbol{\BFi}{\mathalpha}{boperators}{`i}
\DeclareMathSymbol{\BFj}{\mathalpha}{boperators}{`j}
\DeclareMathSymbol{\BFk}{\mathalpha}{boperators}{`k}
\DeclareMathSymbol{\BFl}{\mathalpha}{boperators}{`l}
\DeclareMathSymbol{\BFm}{\mathalpha}{boperators}{`m}
\DeclareMathSymbol{\BFn}{\mathalpha}{boperators}{`n}
\DeclareMathSymbol{\BFo}{\mathalpha}{boperators}{`o}
\DeclareMathSymbol{\BFp}{\mathalpha}{boperators}{`p}
\DeclareMathSymbol{\BFq}{\mathalpha}{boperators}{`q}
\DeclareMathSymbol{\BFr}{\mathalpha}{boperators}{`r}
\DeclareMathSymbol{\BFs}{\mathalpha}{boperators}{`s}
\DeclareMathSymbol{\BFt}{\mathalpha}{boperators}{`t}
\DeclareMathSymbol{\BFu}{\mathalpha}{boperators}{`u}
\DeclareMathSymbol{\BFv}{\mathalpha}{boperators}{`v}
\DeclareMathSymbol{\BFw}{\mathalpha}{boperators}{`w}
\DeclareMathSymbol{\BFx}{\mathalpha}{boperators}{`x}
\DeclareMathSymbol{\BFy}{\mathalpha}{boperators}{`y}
\DeclareMathSymbol{\BFz}{\mathalpha}{boperators}{`z}
\DeclareMathSymbol{\BFA}{\mathalpha}{boperators}{`A}
\DeclareMathSymbol{\BFB}{\mathalpha}{boperators}{`B}
\DeclareMathSymbol{\BFC}{\mathalpha}{boperators}{`C}
\DeclareMathSymbol{\BFD}{\mathalpha}{boperators}{`D}
\DeclareMathSymbol{\BFE}{\mathalpha}{boperators}{`E}
\DeclareMathSymbol{\BFF}{\mathalpha}{boperators}{`F}
\DeclareMathSymbol{\BFG}{\mathalpha}{boperators}{`G}
\DeclareMathSymbol{\BFH}{\mathalpha}{boperators}{`H}
\DeclareMathSymbol{\BFI}{\mathalpha}{boperators}{`I}
\DeclareMathSymbol{\BFJ}{\mathalpha}{boperators}{`J}
\DeclareMathSymbol{\BFK}{\mathalpha}{boperators}{`K}
\DeclareMathSymbol{\BFL}{\mathalpha}{boperators}{`L}
\DeclareMathSymbol{\BFM}{\mathalpha}{boperators}{`M}
\DeclareMathSymbol{\BFN}{\mathalpha}{boperators}{`N}
\DeclareMathSymbol{\BFO}{\mathalpha}{boperators}{`O}
\DeclareMathSymbol{\BFP}{\mathalpha}{boperators}{`P}
\DeclareMathSymbol{\BFQ}{\mathalpha}{boperators}{`Q}
\DeclareMathSymbol{\BFR}{\mathalpha}{boperators}{`R}
\DeclareMathSymbol{\BFS}{\mathalpha}{boperators}{`S}
\DeclareMathSymbol{\BFT}{\mathalpha}{boperators}{`T}
\DeclareMathSymbol{\BFU}{\mathalpha}{boperators}{`U}
\DeclareMathSymbol{\BFV}{\mathalpha}{boperators}{`V}
\DeclareMathSymbol{\BFW}{\mathalpha}{boperators}{`W}
\DeclareMathSymbol{\BFX}{\mathalpha}{boperators}{`X}
\DeclareMathSymbol{\BFY}{\mathalpha}{boperators}{`Y}
\DeclareMathSymbol{\BFZ}{\mathalpha}{boperators}{`Z}
%
\DeclareMathSymbol{\BFzero}{\mathalpha}{boperators}{`0}
\DeclareMathSymbol{\BFone}{\mathalpha}{boperators}{`1}
\DeclareMathSymbol{\BFtwo}{\mathalpha}{boperators}{`2}
\DeclareMathSymbol{\BFthree}{\mathalpha}{boperators}{`3}
\DeclareMathSymbol{\BFfour}{\mathalpha}{boperators}{`4}
\DeclareMathSymbol{\BFfive}{\mathalpha}{boperators}{`5}
\DeclareMathSymbol{\BFsix}{\mathalpha}{boperators}{`6}
\DeclareMathSymbol{\BFseven}{\mathalpha}{boperators}{`7}
\DeclareMathSymbol{\BFeight}{\mathalpha}{boperators}{`8}
\DeclareMathSymbol{\BFnine}{\mathalpha}{boperators}{`9}
%
\DeclareMathSymbol{\BFalpha}{\mathord}{bletters}{"0B}
\DeclareMathSymbol{\BFbeta}{\mathord}{bletters}{"0C}
\DeclareMathSymbol{\BFgamma}{\mathord}{bletters}{"0D}
\DeclareMathSymbol{\BFdelta}{\mathord}{bletters}{"0E}
\DeclareMathSymbol{\BFepsilon}{\mathord}{bletters}{"0F}
\DeclareMathSymbol{\BFzeta}{\mathord}{bletters}{"10}
\DeclareMathSymbol{\BFeta}{\mathord}{bletters}{"11}
\DeclareMathSymbol{\BFtheta}{\mathord}{bletters}{"12}
\DeclareMathSymbol{\BFiota}{\mathord}{bletters}{"13}
\DeclareMathSymbol{\BFkappa}{\mathord}{bletters}{"14}
\DeclareMathSymbol{\BFlambda}{\mathord}{bletters}{"15}
\DeclareMathSymbol{\BFmu}{\mathord}{bletters}{"16}
\DeclareMathSymbol{\BFnu}{\mathord}{bletters}{"17}
\DeclareMathSymbol{\BFxi}{\mathord}{bletters}{"18}
\DeclareMathSymbol{\BFpi}{\mathord}{bletters}{"19}
\DeclareMathSymbol{\BFrho}{\mathord}{bletters}{"1A}
\DeclareMathSymbol{\BFsigma}{\mathord}{bletters}{"1B}
\DeclareMathSymbol{\BFtau}{\mathord}{bletters}{"1C}
\DeclareMathSymbol{\BFupsilon}{\mathord}{bletters}{"1D}
\DeclareMathSymbol{\BFphi}{\mathord}{bletters}{"1E}
\DeclareMathSymbol{\BFchi}{\mathord}{bletters}{"1F}
\DeclareMathSymbol{\BFpsi}{\mathord}{bletters}{"20}
\DeclareMathSymbol{\BFomega}{\mathord}{bletters}{"21}
\DeclareMathSymbol{\BFvarepsilon}{\mathord}{bletters}{"22}
\DeclareMathSymbol{\BFvartheta}{\mathord}{bletters}{"23}
\DeclareMathSymbol{\BFvarpi}{\mathord}{bletters}{"24}
\DeclareMathSymbol{\BFvarrho}{\mathord}{bletters}{"25}
\DeclareMathSymbol{\BFvarsigma}{\mathord}{bletters}{"26}
\DeclareMathSymbol{\BFvarphi}{\mathord}{bletters}{"27}
\DeclareMathSymbol{\BFGamma}{\mathalpha}{boperators}{"00}
\DeclareMathSymbol{\BFDelta}{\mathalpha}{boperators}{"01}
\DeclareMathSymbol{\BFTheta}{\mathalpha}{boperators}{"02}
\DeclareMathSymbol{\BFLambda}{\mathalpha}{boperators}{"03}
\DeclareMathSymbol{\BFXi}{\mathalpha}{boperators}{"04}
\DeclareMathSymbol{\BFPi}{\mathalpha}{boperators}{"05}
\DeclareMathSymbol{\BFSigma}{\mathalpha}{boperators}{"06}
\DeclareMathSymbol{\BFUpsilon}{\mathalpha}{boperators}{"07}
\DeclareMathSymbol{\BFPhi}{\mathalpha}{boperators}{"08}
\DeclareMathSymbol{\BFPsi}{\mathalpha}{boperators}{"09}
\DeclareMathSymbol{\BFOmega}{\mathalpha}{boperators}{"0A}
\DeclareMathSymbol{\BFimath}{\mathord}{bletters}{"7B}
\DeclareMathSymbol{\BFjmath}{\mathord}{bletters}{"7C}
\DeclareMathSymbol{\BFell}{\mathord}{bletters}{"60}
\DeclareMathSymbol{\BFwp}{\mathord}{bletters}{"7D}
\DeclareMathSymbol{\BFnabla}{\mathord}{bsymbols}{"72}
%
\DeclareSymbolFontAlphabet{\BFcal}{bsymbols}
%
\DeclareMathSymbol{\BFcalA}{\mathalpha}{bsymbols}{`A}
\DeclareMathSymbol{\BFcalB}{\mathalpha}{bsymbols}{`B}
\DeclareMathSymbol{\BFcalC}{\mathalpha}{bsymbols}{`C}
\DeclareMathSymbol{\BFcalD}{\mathalpha}{bsymbols}{`D}
\DeclareMathSymbol{\BFcalE}{\mathalpha}{bsymbols}{`E}
\DeclareMathSymbol{\BFcalF}{\mathalpha}{bsymbols}{`F}
\DeclareMathSymbol{\BFcalG}{\mathalpha}{bsymbols}{`G}
\DeclareMathSymbol{\BFcalH}{\mathalpha}{bsymbols}{`H}
\DeclareMathSymbol{\BFcalI}{\mathalpha}{bsymbols}{`I}
\DeclareMathSymbol{\BFcalJ}{\mathalpha}{bsymbols}{`J}
\DeclareMathSymbol{\BFcalK}{\mathalpha}{bsymbols}{`K}
\DeclareMathSymbol{\BFcalL}{\mathalpha}{bsymbols}{`L}
\DeclareMathSymbol{\BFcalM}{\mathalpha}{bsymbols}{`M}
\DeclareMathSymbol{\BFcalN}{\mathalpha}{bsymbols}{`N}
\DeclareMathSymbol{\BFcalO}{\mathalpha}{bsymbols}{`O}
\DeclareMathSymbol{\BFcalP}{\mathalpha}{bsymbols}{`P}
\DeclareMathSymbol{\BFcalQ}{\mathalpha}{bsymbols}{`Q}
\DeclareMathSymbol{\BFcalR}{\mathalpha}{bsymbols}{`R}
\DeclareMathSymbol{\BFcalS}{\mathalpha}{bsymbols}{`S}
\DeclareMathSymbol{\BFcalT}{\mathalpha}{bsymbols}{`T}
\DeclareMathSymbol{\BFcalU}{\mathalpha}{bsymbols}{`U}
\DeclareMathSymbol{\BFcalV}{\mathalpha}{bsymbols}{`V}
\DeclareMathSymbol{\BFcalW}{\mathalpha}{bsymbols}{`W}
\DeclareMathSymbol{\BFcalX}{\mathalpha}{bsymbols}{`X}
\DeclareMathSymbol{\BFcalY}{\mathalpha}{bsymbols}{`Y}
\DeclareMathSymbol{\BFcalZ}{\mathalpha}{bsymbols}{`Z}
%************************-e-bold math letters
%
\DeclareMathSizes{8.0}{8.0}{5.0}{5.0}%
\DeclareMathSizes{9.0}{9.0}{6.0}{5.0}%
\DeclareMathSizes{10.0}{10.0}{6.5}{5.0}% footnotes; references; quotes; tables
\DeclareMathSizes{11.0}{11.0}{7.0}{6.0}% appendix (in most cases)
\DeclareMathSizes{12.0}{12.0}{8.0}{6.0}% regular text; \subsubsection (and below)
\DeclareMathSizes{13.0}{13.0}{9.0}{7.0}% \subsection size
\DeclareMathSizes{14.0}{14.0}{9.0}{7.0}% \section size
\DeclareMathSizes{20.0}{20.0}{14.0}{10.0}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%-e-from-ffi-ti01(modified)

%%%=============================================================================
%%% CROPMARKS
\newdimen\markwidth
\newdimen\blth
\newdimen\marklength
\newdimen\markdistance
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\auxaaa
\newdimen\auxbbb
\newdimen\auxccc
\newdimen\auxddd
\markwidth=.5pt %0.4 truept % Thickness of the mark line
\blth=0.2pt
\marklength=20 truept % Length of the mark line
\markdistance=3 truept % Distance of the real corner to the beg. of the mark
\auxaaa\marklength\advance\auxaaa\markdistance
\def\oddevenswitch{\ifodd\c@page \auxbbb=\oddsidemargin
 \else\auxbbb=\evensidemargin\fi}%
\def\PagePositionCropYes#1#2#3#4#5#6#7#8{%
  \oddsidemargin=#1%
  \evensidemargin=#2%
  \topmargin=#3%
  \headheight=#4%
  \trimwidth=#5%
  \trimheight=#6%
  \hoffset=#7%
  \voffset=#8%
%%%
 \def\CROPMARKS{\oddevenswitch
 \hbox to0pt{\kern-\auxbbb
   \vbox to0bp{\kern-\topmargin\kern-\headheight
   \hbox to\trimwidth{%
     \koo{-\auxaaa}{-\markwidth}{\VRHDW{\markwidth}{0pt}{\marklength}}%
     \koo{-\markwidth}{-\auxaaa}{\VRHDW{0pt}{\marklength}{\markwidth}}%
     \hfill
     \koo{\markdistance}{-\markwidth}{\VRHDW{\markwidth}{0pt}{\marklength}}%
     \koo{0pt}{-\auxaaa}{\VRHDW{0pt}{\marklength}{\markwidth}}}%
   \nointerlineskip\vskip\trimheight
   \nointerlineskip
   \hbox to\trimwidth{%
     \koo{-\auxaaa}{0pt}{\VRHDW{0pt}{\markwidth}{\marklength}}%
     \koo{-\markwidth}{\markdistance}{\VRHDW{0pt}{\marklength}{\markwidth}}%
     \hfill
     \koo{\markdistance}{0pt}{\VRHDW{0pt}{\markwidth}{\marklength}}%
     \koo{0pt}{\markdistance}{\VRHDW{0pt}{\marklength}{\markwidth}}}%
   \vss}\hss}}%
}%

\def\PagePositionCropNo#1#2#3#4#5#6#7#8{%
  \oddsidemargin=#1%  % [3] inner margin / gutter
  \evensidemargin=#2% % [4] outside margin
  \topmargin=#3%      % [5] \rhsink = \topmargin + \headheight (=12pt here)
  \headheight=#4%     % [6] VERY IMPORTANT! (see above)
  \trimwidth=#5%      % [7]
  \trimheight=#6%     % [8]
  \hoffset=#7%        % = -1in to move the area in the upper left corner
  \voffset=#8%        % = -1in to move the area in the upper left corner
%%%
\def\CROPMARKS{}%
}%

\def\PagePositionBoxYes#1#2#3#4#5#6#7#8{%
  \oddsidemargin=#1%  % [3] inner margin / gutter
  \evensidemargin=#2% % [4] outside margin
  \topmargin=#3%      % [5] \rhsink = \topmargin + \headheight (=12pt here)
  \headheight=#4%     % [6] VERY IMPORTANT! (see above)
  \trimwidth=#5%      % [7]
  \trimheight=#6%     % [8]
  \hoffset=#7%        % = -1in to move the area in the upper left corner
  \voffset=#8%        % = -1in to move the area in the upper left corner
%%%
 \def\CROPMARKS{\oddevenswitch
 \hbox to0pt{\kern-\auxbbb
   \vbox to0bp{\kern-\topmargin\kern-\headheight
   \hbox to\trimwidth{%
     \auxccc=\trimwidth \advance\auxccc by 2\blth
     \auxddd=\trimheight \advance\auxddd by 2\blth
     \koo{-\blth}{0pt}{\zeroLL{\VRHDW{\blth}{0pt}{\auxccc}}}%
     \koo{-\blth}{-\blth}{\zeroUL{\VRHDW{\auxddd}{0pt}{\blth}}}%
     \koo{\trimwidth}{-\blth}{\zeroUL{\VRHDW{\auxddd}{0pt}{\blth}}}%
     \koo{-\blth}{\trimheight}{\zeroUL{\VRHDW{\blth}{0pt}{\auxccc}}}\hss}%
   \vss}\hss}}%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end_CROPMARKS

\newcommand\@ptsize{}
\newif\if@restonecol
\newif\if@titlepage\@titlepagefalse
\newif\if@nameyear\@nameyearfalse
%%% PAPER SIZE
\DeclareOption{letterpaper}
   {\setlength\paperheight{11in}\setlength\paperwidth{8.5in}}
\DeclareOption{nameyear}{\@nameyeartrue}
\DeclareOption{oneside}{\@twosidefalse \@mparswitchfalse}
\DeclareOption{twoside}{\@twosidetrue  \@mparswitchtrue}
\DeclareOption{onecolumn}{\@twocolumnfalse}
\DeclareOption{twocolumn}{\@twocolumntrue}
%%% TRIM options
\DeclareOption{draft}{\setlength\overfullrule{5pt}%
  \AtBeginDocument{\PagePositionCropYes
    {72bp}{72bp}{36bp}{28bp}
    {8.5in}{11in}{-1in}{-1in}}}
\DeclareOption{final}{\setlength\overfullrule{0pt}%
  \AtBeginDocument{\PagePositionCropNo
    {72bp}{72bp}{36bp}{28bp}
    {8.5in}{11in}{-1in}{-1in}}}
\DeclareOption{finalbox}{\setlength\overfullrule{0pt}%
  \AtBeginDocument{\PagePositionBoxYes
    {72bp}{72bp}{36bp}{28bp}
    {8.5in}{11in}{-1in}{-1in}}}
%%% end_TRIM options
\newcounter{nowappendix}
\setcounter{nowappendix}{0}%
%%% Journal options (Exactly ONE must be declared as option)
\newif\if@DECA\@DECAfalse
\newif\if@IJOC\@IJOCfalse
\newif\if@INTE\@INTEfalse
\newif\if@ISRE\@ISREfalse
\newif\if@MNSC\@MNSCfalse
\newif\if@MKSC\@MKSCfalse
\newif\if@MOOR\@MOORfalse
\newif\if@MSOM\@MSOMfalse
\newif\if@OPRE\@OPREfalse
\newif\if@ORSC\@ORSCfalse
\newif\if@TRSC\@TRSCfalse
\newif\if@ITED\@ITEDfalse
\DeclareOption{deca}{\@DECAtrue}
\DeclareOption{ijoc}{\@IJOCtrue}
\DeclareOption{inte}{\@INTEtrue}
\DeclareOption{isre}{\@ISREtrue}
\DeclareOption{mnsc}{\@MNSCtrue}
\DeclareOption{mksc}{\@MKSCtrue}
\DeclareOption{moor}{\@MOORtrue}
\DeclareOption{msom}{\@MSOMtrue}
\DeclareOption{opre}{\@OPREtrue}
\DeclareOption{orsc}{\@ORSCtrue}
\DeclareOption{trsc}{\@TRSCtrue}
\DeclareOption{ited}{\@ITEDtrue}
%
\newif\if@COPYEDIT\@COPYEDITfalse
\DeclareOption{copyedit}{\@COPYEDITtrue}
%
\newif\if@BLINDREV\@BLINDREVfalse
\DeclareOption{blindrev}{\@BLINDREVtrue}
%
\newif\if@NONBLINDREV\@NONBLINDREVfalse
\DeclareOption{nonblindrev}{\@NONBLINDREVtrue}
%
\newif\if@BIGACK\@BIGACKfalse
\def\bigack{\@BIGACKtrue}
%
\DeclareOption{openbib}{%
  \AtEndOfPackage{%
   \renewcommand\@openbib@code{%
      \advance\leftmargin\bibindent
      \itemindent -\bibindent
      \listparindent \itemindent
      \parsep \z@
      }%
   \renewcommand\newblock{\par}}%
}
\ExecuteOptions{letterpaper,twoside,onecolumn,final}
\ProcessOptions
%****************************************************************************

%%%%%%%%%%%%%%%%%FFF

%%%\input{04set01.sty} % general settings of most parameters
%%%%%%%%%%%%%%%%%%%%%%-b-Standard sizes and their versions
\newdimen\@bls \@bls=13.2pt
\newdimen\@em \@em=11pt

\def\fs.#1.#2.{\fontsize{#1}{#2}\selectfont}%

\def\Dskips#1#2#3#4{\abovedisplayskip #1em \@plus#2em \@minus#3em
   \abovedisplayshortskip \z@ \@plus#2em
   \belowdisplayshortskip #4em \@plus#2em \@minus#2em
   \belowdisplayskip \abovedisplayskip}%
% standard 10pt is \Dskips{10}{3}{5}{6}%
\Dskips{1.0}{0.3}{0.5}{0.6}%


\newcommand\TEN{\relax}%
\newcommand\NIN{\relax}%
\newcommand\EGT{\relax}%
%\newcommand\normalsize{\relax}%
\newcommand\small{\relax}%
\newcommand\footnotesize{\relax}%

\def\SingleSpacedXI{%
\renewcommand\TEN{\normalsizeXInoCE}%
\renewcommand\NIN{\smallXnoCE}%
\renewcommand\EGT{\footnotesizeIXnoCE}%
\renewcommand\normalsize{\normalsizeXInoCE}%
\renewcommand\small{\smallXnoCE}%
\renewcommand\footnotesize{\footnotesizeIXnoCE}%
\normalsizeXInoCE
}

\def\DoubleSpacedXI{%
\renewcommand\TEN{\normalsizeXIyesCE}%
\renewcommand\NIN{\smallXyesCE}%
\renewcommand\EGT{\footnotesizeIXyesCE}%
\renewcommand\normalsize{\normalsizeXIyesCE}%
\renewcommand\small{\smallXyesCE}%
\renewcommand\footnotesize{\footnotesizeIXyesCE}%
\normalsizeXIyesCE
}

\def\SingleSpacedXII{%
\renewcommand\TEN{\normalsizeXIInoCE}%
\renewcommand\NIN{\smallXnoCE}%
\renewcommand\EGT{\footnotesizeIXnoCE}%
\renewcommand\normalsize{\normalsizeXIInoCE}%
\renewcommand\small{\smallXnoCE}%
\renewcommand\footnotesize{\footnotesizeIXnoCE}%
\normalsizeXIInoCE
}

\def\DoubleSpacedXII{%
\renewcommand\TEN{\normalsizeXIIyesCE}%
\renewcommand\NIN{\smallXyesCE}%
\renewcommand\EGT{\footnotesizeIXyesCE}%
\renewcommand\normalsize{\normalsizeXIIyesCE}%
\renewcommand\small{\smallXyesCE}%
\renewcommand\footnotesize{\footnotesizeIXyesCE}%
\normalsizeXIIyesCE
}

\def\OneAndAHalfSpacedXII{%
\renewcommand\TEN{\AAnormalsizeXII}%
\renewcommand\NIN{\AAsmallX}%
\renewcommand\EGT{\AAfootnotesizeIX}%
\renewcommand\normalsize{\AAnormalsizeXII}%
\renewcommand\small{\AAsmallX}%
\renewcommand\footnotesize{\AAfootnotesizeIX}%
\AAnormalsizeXII
}

\def\OneAndAHalfSpacedXI{%
\renewcommand\TEN{\AAnormalsizeXI}%
\renewcommand\NIN{\AAsmallX}%
\renewcommand\EGT{\AAfootnotesizeIX}%
\renewcommand\normalsize{\AAnormalsizeXI}%
\renewcommand\small{\AAsmallX}%
\renewcommand\footnotesize{\AAfootnotesizeIX}%
\AAnormalsizeXI
}

\def\TableSpaced{%
\renewcommand\TEN{\TABLEnormalsizeXI}%
\renewcommand\NIN{\TABLEsmallX}%
\renewcommand\EGT{\TABLEfootnotesizeIX}%
\renewcommand\normalsize{\TABLEnormalsizeXI}%
\renewcommand\small{\TABLEsmallX}%
\renewcommand\footnotesize{\TABLEfootnotesizeIX}%
\TABLEnormalsizeXI
}

\newcommand\AAnormalsizeXII{%
   \@setfontsize\normalsizeXI{12}{20.7}%
   \Dskips{1.0}{0.3}{0.5}{0.6}%
   \let\@listi\@listI
   \baselineskip20.7pt plus 1pt minus 1pt
\@bls=20.7pt\@em=12pt
\relax}

\newcommand\AAnormalsizeXI{%
   \@setfontsize\normalsizeXI{11}{12.66}%
   \Dskips{1.0}{0.3}{0.5}{0.6}%
   \let\@listi\@listI
   \baselineskip19pt plus 1pt minus 1pt
\@bls=19pt\@em=11pt
\relax}

\newcommand\AAsmallX{%
   \@setfontsize\smallX{10}{11.5}%
   \Dskips{0.8}{0.3}{0.5}{0.6}%
   \def\@listi{\leftmargin\leftmargini
     \topsep 0\p@ \parsep 2\p@ \itemsep \parsep}%
   \baselineskip17.25pt plus 1pt minus 1pt
\@bls=17.25pt\@em=10pt
\relax}

\newcommand\AAfootnotesizeIX{%
   \@setfontsize\footnotesizeIX\@ixpt\@xipt
   \Dskips{0.8}{0.3}{0.5}{0.6}%
   \def\@listi{\leftmargin\leftmargini
      \topsep 0\p@ \parsep 0\p@ \itemsep \parsep}%
   \baselineskip15.5pt plus 1pt minus 1pt
\@bls=15.5pt\@em=9pt
\relax}

\newcommand\normalsizeXIInoCE{%
   \@setfontsize\normalsizeXI{12}{13.80}%
   \Dskips{1.0}{0.3}{0.5}{0.6}%
   \let\@listi\@listI
   \baselineskip13.80pt plus 0.6pt minus 0.4pt
\@bls=13.80pt\@em=12pt
\relax}

\newcommand\normalsizeXInoCE{%
   \@setfontsize\normalsizeXI{11}{12.66}%
   \Dskips{1.0}{0.3}{0.5}{0.6}%
   \let\@listi\@listI
   \baselineskip12.66pt plus 0.6pt minus 0.4pt
\@bls=12.66pt\@em=11pt
\relax}

\newcommand\smallXnoCE{%
   \@setfontsize\smallX{10}{11.5}%
   \Dskips{0.8}{0.3}{0.5}{0.6}%
   \def\@listi{\leftmargin\leftmargini
     \topsep 0\p@ \parsep 2\p@ \itemsep \parsep}%
   \baselineskip11.5pt plus 0.5pt minus 0.35pt
\@bls=11.5pt\@em=10pt
\relax}

\newcommand\footnotesizeIXnoCE{%
   \@setfontsize\footnotesizeIX{9}{10.35}%
   \Dskips{0.8}{0.3}{0.5}{0.6}%
   \def\@listi{\leftmargin\leftmargini
      \topsep 0\p@ \parsep 0\p@ \itemsep \parsep}%
   \baselineskip10.35pt plus 0.4pt minus 0.3pt
\@bls=10.35pt\@em=9pt
\relax}

\newcommand\normalsizeXIIyesCE{%
   \@setfontsize\normalsizeXI{12}{27.6}%
   \Dskips{1.0}{0.3}{0.5}{0.6}%
   \let\@listi\@listI
   \baselineskip27.6pt plus 1pt minus 2pt
\@bls=27.6pt\@em=12pt
\relax}

\newcommand\normalsizeXIyesCE{%
   \@setfontsize\normalsizeXI{11}{25.32}%
   \Dskips{1.0}{0.3}{0.5}{0.6}%
   \let\@listi\@listI
   \baselineskip25.32pt plus 1pt minus 2pt
\@bls=25.32pt\@em=11pt
\relax}

\newcommand\smallXyesCE{%
   \@setfontsize\smallX{10}{23}%
   \Dskips{0.8}{0.3}{0.5}{0.6}%
   \def\@listi{\leftmargin\leftmargini
     \topsep 0\p@ \parsep 2\p@ \itemsep \parsep}%
   \baselineskip23pt plus 1pt minus 1pt
\@bls=23pt\@em=10pt
\relax}

\newcommand\footnotesizeIXyesCE{%
   \@setfontsize\footnotesizeIX{9}{20.7}
   \Dskips{0.8}{0.3}{0.5}{0.6}%
   \def\@listi{\leftmargin\leftmargini
      \topsep 0\p@ \parsep 0\p@ \itemsep \parsep}%
   \baselineskip20.7pt plus 1pt minus 1pt
\@bls=20.7pt\@em=9pt
\relax}

\newcommand\TABLEnormalsizeXI{%
   \@setfontsize\normalsizeX{10}{12}%
   \Dskips{1.0}{0.3}{0.5}{0.6}%
   \let\@listi\@listI
   \baselineskip12pt plus 0.6pt minus 0.4pt
\@bls=12pt\@em=10pt
\relax}

\newcommand\TABLEsmallX{%
   \@setfontsize\smallX{9}{11}%
   \Dskips{0.8}{0.3}{0.5}{0.6}%
   \def\@listi{\leftmargin\leftmargini
     \topsep 0\p@ \parsep 2\p@ \itemsep \parsep}%
   \baselineskip11pt plus 0.5pt minus 0.35pt
\@bls=11pt\@em=9pt
\relax}

\newcommand\TABLEfootnotesizeIX{%
   \@setfontsize\footnotesizeIX{8}{10}%
   \Dskips{0.8}{0.3}{0.5}{0.6}%
   \def\@listi{\leftmargin\leftmargini
      \topsep 0\p@ \parsep 0\p@ \itemsep \parsep}%
   \baselineskip10pt plus 0.4pt minus 0.3pt
\@bls=10pt\@em=8pt
\relax}



\newcommand\scriptsize{\@setfontsize\scriptsize\@viiipt{9.5}}
\newcommand\tiny{\@setfontsize\tiny\@vipt\@viipt}
\newcommand\large{\@setfontsize\large\@xivpt{18}}
\newcommand\Large{\@setfontsize\Large\@xviipt{22}}
\newcommand\LARGE{\@setfontsize\LARGE\@xxpt{25}}
\newcommand\huge{\@setfontsize\huge\@xxvpt{30}}
\let\Huge=\huge

%\def\TEN{\normalsizeXI}%
%\def\NIN{\smallX}%
%\def\EGT{\footnotesizeIX}%
%
%\def\normalsize{\normalsizeXI}%
%\def\small{\smallX}%
%\def\footnotesize{\footnotesizeIX}%


\if@COPYEDIT
\DoubleSpacedXI
\else
\SingleSpacedXI
\fi

\OneAndAHalfSpacedXI % 12/20/2010

%%%%%%%%%%%%%%%%%%%%%%-e-Standard sizes and their versions

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%-b-KOO
\long\def\koo#1#2#3{\vbox to0pt{\hsize0pt\kern #2\hbox to0pt{\kern
#1{#3}\hss}\vss}}
\long\def\zeroCC#1{\vbox to0pt{\vss\hbox to0pt{\hss #1\hss}\vss}}
\long\def\zeroLC#1{\vbox to0pt{\vss\hbox to0pt{\hss #1\hss}}}
\long\def\zeroUC#1{\vbox to0pt{\hbox to0pt{\hss #1\hss}\vss}}
\long\def\zeroLR#1{\vbox to0pt{\vss\hbox to0pt{\hss #1}}}
\long\def\zeroCR#1{\vbox to0pt{\vss\hbox to0pt{\hss #1}\vss}}
\long\def\zeroUR#1{\vbox to0pt{\hbox to0pt{\hss #1}\vss}}
\long\def\zeroLL#1{\vbox to0pt{\vss\hbox to0pt{#1\hss}}}
\long\def\zeroCL#1{\vbox to0pt{\vss\hbox to0pt{#1\hss}\vss}}
\long\def\zeroUL#1{\vbox to0pt{\hbox to0pt{#1\hss}\vss}}
\def\VRHDW#1#2#3{\vrule height #1 depth #2 width #3}
\def\HRHDW#1#2#3{\hrule height #1 depth #2 width #3}
\def\HD#1#2{\vrule height #1pt depth #2pt width 0pt\relax}
%%%%%%%%%%%%%%%%%%%%%%-e-KOO

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%-b-Center etc redefined
% No extra space above and below
\newenvironment{Center}{\parskip0pt\topsep0pt
  \partopsep0pt\parsep0pt\begin{center}}{\end{center}}
\newenvironment{Flushleft}{\parskip0pt\topsep0pt
  \partopsep0pt\parsep0pt\begin{flushleft}}{\end{flushleft}}
\newenvironment{Flushright}{\parskip0pt\topsep0pt
  \partopsep0pt\parsep0pt\begin{flushright}}{\end{flushright}}
%%%%%%%%%%%%%%%%%%%%%%-e-Center etc redefined

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%-b-Standard sizes and penalties
%\newdimen\@bls
%\@bls=\baselineskip
\bigskipamount=\@bls \@plus 0.333\@bls \@minus 0.333\@bls
\medskipamount=0.5\bigskipamount
\smallskipamount=0.25\bigskipamount
\setlength\maxdepth{4pt}
\setlength\marginparwidth{\z@}
\setlength\marginparsep{1pc}
\columnseprule \z@
%
\newbox\tempbox % for figs and tables
\newdimen\tempdim
\newdimen\tempdimht
%
%\def\FNRULE{\koo{0pt}{-9pt}{\zeroLL{\VRHDW{0.5pt}{0pt}{20pc}}}}%
\setlength\footnotesep{12\p@}
\setlength{\skip\footins}{18\p@ \@plus 6\p@ \@minus 6\p@}
\setlength\floatsep    {18\p@ \@plus 10\p@ \@minus 2\p@}
\setlength\textfloatsep{18\p@ \@plus 10\p@ \@minus 2\p@}
\setlength\intextsep   {18\p@ \@plus 10\p@ \@minus 2\p@}
\setlength\dblfloatsep    {18\p@ \@plus 10\p@ \@minus 2\p@}
\setlength\dbltextfloatsep{18\p@ \@plus 10\p@ \@minus 2\p@}
\setlength\@fptop{0\p@}%%{0\p@ \@plus 1fil}
\setlength\@fpsep{8\p@ \@plus 2fil}
\setlength\@fpbot{0\p@ \@plus 1fil}
\setlength\@dblfptop{0\p@}%%%{0\p@ \@plus 1fil}
\setlength\@dblfpsep{8\p@ \@plus 2fil}
\setlength\@dblfpbot{0\p@ \@plus 1fil}
\setlength\partopsep{2\p@ \@plus 1\p@ \@minus 1\p@}
\setlength\lineskip{0\p@}
\setlength\normallineskip{0\p@}
\lineskiplimit0pt
\renewcommand\baselinestretch{}
\setlength\parskip{\z@}
%
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301
\@beginparpenalty -\@lowpenalty    % Before a list or paragraph environment.
\@endparpenalty   -\@lowpenalty    % After a list or paragraph environment.
\@itempenalty     -\@lowpenalty    % Between list items.
%%% FLOATS %%
\setcounter{topnumber}{5}
\def\topfraction{1.0}%%{0.99}
\def\textfraction{0}%%{0.05}
\def\floatpagefraction{0.9}
\setcounter{bottomnumber}{5}
\def\bottomfraction{1.0}%%{0.99}
\setcounter{totalnumber}{10}
\def\dbltopfraction{1.0}%%{0.99}
\def\dblfloatpagefraction{0.8}
\setcounter{dbltopnumber}{5}
%
%%%-b-PENALTIES
\if@COPYEDIT
\clubpenalty 50
\widowpenalty 50
\predisplaypenalty=100
\interdisplaylinepenalty=0
\displaywidowpenalty=200
\else
\clubpenalty 10000
\widowpenalty 10000
\predisplaypenalty=10000
\interdisplaylinepenalty=100
\displaywidowpenalty 1500
\fi
\postdisplaypenalty 0 %%%500
\interlinepenalty 0
\brokenpenalty 500 % Plain default = 100
\adjdemerits=100 % Plain default = 10000
\linepenalty=10
\doublehyphendemerits=10000
\finalhyphendemerits=5000
\hyphenpenalty=50
\exhyphenpenalty=50
\binoppenalty=150 % 700
\relpenalty=100 % 500
\interfootnotelinepenalty=100
\nulldelimiterspace=1.2pt
\lefthyphenmin=3
\righthyphenmin=3
\emergencystretch=2pc
%
\newdimen\adim
%
%\setlength\arraycolsep{5\p@}
%\setlength\tabcolsep{6\p@}
\arraycolsep 1.8pt
\tabcolsep 4pt
\arrayrulewidth .4pt
\doublerulesep 2pt
\tabbingsep\labelsep
%
\def\thefootnote{\arabic{footnote}}
%
\skip\@mpfootins = \skip\footins
\setlength\fboxsep{3\p@}
\setlength\fboxrule{.4\p@}
\jot=0.3em %(LaTeX standard)% in prod. 0.6em
\topsep10\p@ \@plus2\p@ \@minus5\p@
%%%%%%%%%%%%%%%%%%%%%%-e-Standard sizes and penalties

\newcounter{figure}
\renewcommand\thefigure{\@arabic\c@figure}
\def\fps@figure{tbp}
\def\ftype@figure{1}
\def\ext@figure{lof}
\def\fnum@figure{{Figure\hskip0.3em\thefigure}}%% may be redefined by the particular style
\newenvironment{figure}
  {\let\@makecaption\@makefigurecaption\@float{figure}}
  {\end@float}
\newenvironment{figure*}
  {\let\@makecaption\@makefigurecaption\@dblfloat{figure}}
  {\end@dblfloat}
%
\newcounter{table}
\renewcommand\thetable{\@arabic\c@table}
\def\fps@table{tbp}
\def\ftype@table{2}
\def\ext@table{lot}
\def\fnum@table{Table\hskip0.3em\thetable}%% may be redefined by the particular style
\newenvironment{table}
  {\let\@makecaption\@maketablecaption\@float{table}}
  {\end@float}
\newenvironment{table*}
  {\let\@makecaption\@maketablecaption\@dblfloat{table}}
  {\end@dblfloat}

\newcommand\@pnumwidth{1.55em}
\newcommand\@tocrmarg{2.55em}
\newcommand\@dotsep{4.5}
\setcounter{tocdepth}{3}
\newcommand\tableofcontents{%
    \section*{\contentsname
        \@mkboth{%
           \MakeUppercase\contentsname}{\MakeUppercase\contentsname}}%
    \@starttoc{toc}%
    }
\newcommand*\l@part[2]{%
  \ifnum \c@tocdepth >-2\relax
    \addpenalty\@secpenalty
    \addvspace{2.25em \@plus\p@}%
    \begingroup
      \setlength\@tempdima{3em}%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      {\leavevmode
       \large \bfseries #1\hfil \hb@xt@\@pnumwidth{\hss #2}}\par
       \nobreak
       \if@compatibility
         \global\@nobreaktrue
         \everypar{\global\@nobreakfalse\everypar{}}%
      \fi
    \endgroup
  \fi}
\newcommand*\l@section[2]{%
  \ifnum \c@tocdepth >\z@
    \addpenalty\@secpenalty
    \addvspace{1.0em \@plus\p@}%
    \setlength\@tempdima{1.5em}%
    \begingroup
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      \leavevmode \bfseries
      \advance\leftskip\@tempdima
      \hskip -\leftskip
      #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
    \endgroup
  \fi}
\newcommand*\l@subsection{\@dottedtocline{2}{1.5em}{2.3em}}
\newcommand*\l@subsubsection{\@dottedtocline{3}{3.8em}{3.2em}}
\newcommand*\l@paragraph{\@dottedtocline{4}{7.0em}{4.1em}}
\newcommand*\l@subparagraph{\@dottedtocline{5}{10em}{5em}}
\newcommand\listoffigures{%
    \section*{\listfigurename
      \@mkboth{\MakeUppercase\listfigurename}%
              {\MakeUppercase\listfigurename}}%
    \@starttoc{lof}%
    }
\newcommand*\l@figure{\@dottedtocline{1}{1.5em}{2.3em}}
\newcommand\listoftables{%
    \section*{\listtablename
      \@mkboth{%
          \MakeUppercase\listtablename}{\MakeUppercase\listtablename}}%
    \@starttoc{lot}%
    }
\let\l@table\l@figure
%
% This is to hide footnote rule
\renewcommand\footnoterule{}
%  \kern-3\p@\hrule\@width.4\columnwidth\hrule\@width.175\columnwidth\kern2.6\p@% was
%
\newcommand\contentsname{Contents}
\newcommand\listfigurename{List of Figures}
\newcommand\listtablename{List of Tables}
\newcommand\partname{Part}
\newcommand\indexname{Index}
\newcommand\figurename{Figure}%     <-- to be adjusted per journal
\newcommand\tablename{Table}%       <-- to be adjusted per journal
\newcommand\refname{References}%    <-- to be adjusted per journal
\newcommand\appendixname{Appendix}% <-- to be adjusted per journal
%\newcommand\abstractname{Abstract:}
%
\newcommand\today{}
\edef\today{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}
%
\def\copyright{\raisebox{0.06em}{\textcopyright}}
%
\newcommand{\up}{\VRHDW{1.5em}{0em}{0em}}% for tables (8/10 makes 1em = 8pt)
\newcommand{\down}{\VRHDW{0em}{0.625em}{0em}}%
\def\updown{\up\down}
%
% tightness of math; \mathNN is the LaTeX default (too loose); \mathN is new INFORMS default
\def\mathT{\thickmuskip2mu \thinmuskip1mu \medmuskip=1.5mu\relax}
\let\mathtight=\mathT % pure synonym to \mathT
\let\tightmath=\mathT % pure synonym to \mathT
\def\mathN{\thickmuskip3.5mu plus 2mu\thinmuskip2.5mu\medmuskip=3mu plus 2mu minus 1.5mu\relax}
\def\mathNN{\thickmuskip=5mu plus 5mu\thinmuskip=3mu\medmuskip=4mu plus 2mu minus 4mu\relax}
\mathN %% <-- INFORMS default (tighter than the regular \mathNN)
%
%%% some abbreviations:
\def\0{\phantom{0}}%
\def\Bull{\unskip\hskip0.5em{\textbullet}\hskip0.5em\relax}
\def\COLON{{:}\ }
\def\DS{\displaystyle}
\def\EQNpagebreak{\removelastskip\hrule height0pt\eject}
\def\halmos{\mbox{\quad$\square$}}
\def\Halmos{\mbox{\quad$\square$}}% \square <--> \blackbox (?)
\def\qed{\quad Q.E.D.}
\def\LM{\leavevmode}%
\def\NNN{\nonumber}%
\def\PD{\partial}%
\def\argmax{\mathop{\rm arg\,max}}%
\def\argmin{\mathop{\rm arg\,min}}%
\def\RB#1#2{\raisebox{#1pt}[0pt][0pt]{\tabcolsep0pt\begin{tabular}[b]{c}#2\end{tabular}}}
\def\RBL#1#2{\raisebox{#1pt}[0pt][0pt]{\tabcolsep0pt\begin{tabular}[b]{l}#2\end{tabular}}}
\def\RBX#1#2{\raisebox{#1}[0pt][0pt]{#2}}
\def\SPN{\spaceskip 0.33em plus 0.167em minus 0.09em\relax}% normal values
\def\SPTT{\spaceskip 0.25em plus 0.14em minus 0.06em\relax}
\def\SPT{\spaceskip 0.3em plus 0.16em minus 0.09em\relax}
\def\TS{\textstyle}
\def\bee{\begin{eqnarray}}%
\def\bees{\begin{eqnarray*}}%
\def\be{\begin{equation}}%
\def\eee{\end{eqnarray}}%
\def\eees{\end{eqnarray*}}%
\def\ee{\end{equation}}%
\def\epb{\EQNpagebreak}
\def\hph#1{\hphantom{#1}}
\def\PHE{\hphantom{{}={}}}% useful in alignments
\def\h{\hbox}
\def\mc#1{\multicolumn{1}{c}{#1}}%
\def\mcc#1#2{\multicolumn{#1}{c}{#2}}%
\def\mcr{\\[-0.3em]\\}%%{\\[-0.6em]\\}
\def\mccz#1#2{\multicolumn{#1}{c}{\hbox to 0pt{\hss #2\hss}}}%
\def\mcz#1{\multicolumn{1}{c}{\hbox to 0pt{\hss #1\hss}}}
\def\n{\nobreak}
\def\vs#1{\vadjust{\vspace{#1pt}}}
\def\vvSP#1{\HD{0}{#1}\pagebreak}
\def\vvp{\vadjust{\vfill\pagebreak}}
\def\xxx{\end{document}}
\long\def\IGNORE#1{}
\long\def\IGNORETHIS#1{}%
\def\RAGG{\rightskip0pt plus 1fil}%
\def\HET{\hsize=\textwidth}% for tables and figures 2-col in [b]
\def\BBB{\break}%
\def\PPPP{\pagebreak}%

%%%%%%%% common but adjustable per journal style:
\parindent 1em
%%%\setlength\headheight{60pt} %<-- set by icrops1.sty
\headsep14pt
\topskip 10pt %%
\footskip 0pt % 36pt
\textheight 648pt
\textwidth 6.5in
\columnsep 1.5pc\columnseprule 0pt

\newenvironment{extract}{\begin{list}{}{\NIN
  \topsep\medskipamount
  \leftmargin 1em \rightmargin 1em \parsep 0pt \itemsep 0pt
  \itemindent 0pt \listparindent 1em}\item[]}%
  {\end{list}}

\newcommand\@makefntext[1]{\parindent 1em\noindent\ignorespaces{\@makefnmark}\,#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%-article-opening-etc

\newif\iftitle
\global\titlefalse

\def\JOURNAL#1{\gdef\theJOURNAL{#1}}\def\theJOURNAL{Journal Name}%
\def\VOLUME#1{\gdef\theVOLUME{#1}}\def\theVOLUME{00}%
\def\NO#1{\gdef\theNO{#1}}\def\theNO{0}%
\def\ISSUE#1{\gdef\theISSUE{#1}}\def\theISSUE{0000}% default
\def\MONTH#1{\gdef\theMONTH{#1}}\def\theMONTH{Xxxxx}%
\def\YEAR#1{\gdef\theYEAR{#1}}\def\theYEAR{0000}% default
\def\ISSN#1{\gdef\theISSN{#1}}\def\theISSN{0000-0000}% default
\def\EISSN#1{\gdef\theEISSN{#1}}\def\theEISSN{0000-0000}% default
\def\DOI#1{\gdef\theDOI{#1}}\def\theDOI{10.1287/xxxx.0000.0000}% default
\def\FIRSTPAGE#1{\gdef\theFIRSTPAGE{#1}}\def\theFIRSTPAGE{000}%
\def\LONGFIRSTPAGE#1{\gdef\theLONGFIRSTPAGE{#1}}\def\theLONGFIRSTPAGE{0001}% default
\def\LASTPAGE#1{\gdef\theLASTPAGE{#1}}\def\theLASTPAGE{000}%
\def\SHORTYEAR#1{\gdef\theSHORTYEAR{#1}}\def\theSHORTYEAR{00}% default
\def\PAGERANGE#1{\gdef\thePAGERANGE{#1}}\def\thePAGERANGE{}%
\def\TITLE#1{\gdef\theTITLE{#1}}\def\theTITLE{}%{Article Title}%
\def\RUNAUTHOR#1{\gdef\theRUNAUTHOR{#1}}\def\theRUNAUTHOR{Author}% default
\def\RUNTITLE#1{\gdef\theRUNTITLE{#1}}\def\theRUNTITLE{Article Short Title}% default
\def\ECRUNAUTHOR#1{\gdef\theECRUNAUTHOR{#1}}\def\theECRUNAUTHOR{\theRUNAUTHOR}% default
\def\ECRUNTITLE#1{\gdef\theECRUNTITLE{#1}}\def\theECRUNTITLE{\theRUNTITLE}% default
\def\ECTYPE#1{\gdef\theECTYPE{#1}}\def\theECTYPE{e-companion to\enspace}% default
\def\ECAUpunct#1{\gdef\theECAUpunct{#1}}\def\theECAUpunct{:\space}% default


\def\LRHFirstLine#1{\gdef\theLRHFirstLine{#1}}\def\theLRHFirstLine{}%
\def\LRHSecondLine#1{\gdef\theLRHSecondLine{#1}}\def\theLRHSecondLine{}%
\def\RRHFirstLine#1{\gdef\theRRHFirstLine{#1}}\def\theRRHFirstLine{}%
\def\RRHSecondLine#1{\gdef\theRRHSecondLine{#1}}\def\theRRHSecondLine{}%

\def\ECLRHFirstLine#1{\gdef\theECLRHFirstLine{#1}}\def\theECLRHFirstLine{}%
\def\ECLRHSecondLine#1{\gdef\theECLRHSecondLine{#1}}\def\theECLRHSecondLine{}%
\def\ECRRHFirstLine#1{\gdef\theECRRHFirstLine{#1}}\def\theECRRHFirstLine{}%
\def\ECRRHSecondLine#1{\gdef\theECRRHSecondLine{#1}}\def\theECRRHSecondLine{}%

\def\LRFFirstLine#1{\gdef\theLRFFirstLine{#1}}\def\theLRFFirstLine{}%
\def\LRFSecondLine#1{\gdef\theLRFSecondLine{#1}}\def\theLRFSecondLine{}%
\def\RRFFirstLine#1{\gdef\theRRFFirstLine{#1}}\def\theRRFFirstLine{}%
\def\RRFSecondLine#1{\gdef\theRRFSecondLine{#1}}\def\theRRFSecondLine{}%

\if@BLINDREV
\long\def\ARTICLEAUTHORS#1{\gdef\theARTICLEAUTHORS{%
  \begin{Center}\HOOKa\vspace*{0pt}{\fs.12.12.\bf (Authors' names blinded for peer review)}\vspace*{0pt}\end{Center}}}%
\else
\long\def\ARTICLEAUTHORS#1{\gdef\theARTICLEAUTHORS{%
  \begin{Center}\HOOKa\vspace*{0pt}#1\vspace*{0pt}\end{Center}}}%
\fi
\def\theARTICLEAUTHORS{}%

\long\def\ABSTRACT#1{\long\gdef\theABSTRACT{#1}}\def\theABSTRACT{}%

\def\SEPBAR{$\mskip2.5mu|\mskip2.5mu$}

\def\SUBJECTCLASSname{{\it Subject classifications\/}{\kern0.7pt}:\enskip}
\def\AREAOFREVIEWname{{\it Area of review\/}{\kern0.7pt}:\enskip}
\def\HISTORYname{{\it History\/}{\kern0.7pt}:\enskip}
\def\MSCCLASSname{{\it MSC2000 subject classification\/}{\kern0.7pt}:\enskip}
\def\ORMSCLASSname{{\it OR/MS subject classification\/}{\kern0.7pt}:\enskip}
\def\KEYWORDSname{{\it Key words\/}{\kern0.7pt}:\enskip}

\def\HISTORY#1{\gdef\theHISTORY{\endgraf\rightskip0pt plus 20pc
  \noindent\hangindent1em\HISTORYname #1\endgraf}}\def\theHISTORY{}%
\def\AREAOFREVIEW#1{\gdef\theAREAOFREVIEW{\endgraf\rightskip0pt plus 20pc
  \noindent\hangindent1em\AREAOFREVIEWname #1\endgraf}}\def\theAREAOFREVIEW{}%
\def\SUBJECTCLASS#1{\gdef\theSUBJECTCLASS{\endgraf\rightskip0pt plus 20pc
  \noindent\hangindent1em\SUBJECTCLASSname #1\endgraf}}\def\theSUBJECTCLASS{}%
\def\MSCCLASS#1{\gdef\theMSCCLASS{\endgraf\rightskip0pt plus 20pc
  \noindent\hangindent1em\MSCCLASSname #1\endgraf}}\def\theMSCCLASS{}%
\def\ORMSCLASS#1{\gdef\theORMSCLASS{\endgraf\rightskip0pt plus 20pc
  \noindent\hangindent1em\ORMSCLASSname #1\endgraf}}\def\theORMSCLASS{}%
\def\KEYWORDS#1{\gdef\theKEYWORDS{\endgraf\rightskip0pt plus 20pc
  \noindent\hangindent1em\KEYWORDSname #1\endgraf}}\def\theKEYWORDS{}%
\def\thePAGERANGE{pp.~\theFIRSTPAGE--\theLASTPAGE}% default
\def\theRUNPAGERANGE{pp.~\theFIRSTPAGE--\theLASTPAGE}% default

%%% pagestyles revised:

\def\setoddRF{\hfil} \def\setevenRF{\hfil} % Running feet empty

\def\setoddRH{\hbox to \textwidth{\fs.7.8.\tabcolsep0pt
  \begin{tabular*}{\textwidth}[b]{l@{\extracolsep\fill}r}
  {\theRRHFirstLine}&\\ {\theRRHSecondLine}&  \raisebox{0pt}[0pt][0pt]{\fs.10.10.\thepage}\\[-4pt]
  \rlap{\VRHDW{0.5pt}{0pt}{\textwidth}}&\\
  \end{tabular*}}}
\def\setevenRH{\hbox to \textwidth{\fs.7.8.\tabcolsep0pt
  \begin{tabular*}{\textwidth}[b]{l@{\extracolsep\fill}r}
  &{\theLRHFirstLine}\\ \raisebox{0pt}[0pt][0pt]{\fs.10.10.\thepage}&{\theLRHSecondLine}\\[-4pt]
  \rlap{\VRHDW{0.5pt}{0pt}{\textwidth}}&\\
  \end{tabular*}}}

\RRHFirstLine{\bf\theRUNAUTHOR:\enskip {\it\theRUNTITLE}}% default
\RRHSecondLine{\fs.7.9.{\theJOURNAL} \theVOLUME(\theNO), \theRUNPAGERANGE,
  \copyright\,{\theYEAR}\ INFORMS}% default
\LRHFirstLine{\bf\theRUNAUTHOR:\enskip {\it\theRUNTITLE}}% default
\LRHSecondLine{\fs.7.9.{\theJOURNAL} \theVOLUME(\theNO), \theRUNPAGERANGE,
  \copyright\,{\theYEAR}\ INFORMS}% default

\def\setoddECRH{\hbox to \textwidth{\fs.7.8.\tabcolsep0pt
  \begin{tabular*}{\textwidth}[b]{l@{\extracolsep\fill}r}
  {\theECRRHFirstLine}&\\ {\theECRRHSecondLine}&  \raisebox{0pt}[0pt][0pt]{\fs.10.10.\thepage}\\[-4pt]
  \rlap{\VRHDW{0.5pt}{0pt}{\textwidth}}&\\
  \end{tabular*}}}
\def\setevenECRH{\hbox to \textwidth{\fs.7.8.\tabcolsep0pt
  \begin{tabular*}{\textwidth}[b]{l@{\extracolsep\fill}r}
  &{\theECLRHFirstLine}\\ \raisebox{0pt}[0pt][0pt]{\fs.10.10.\thepage}&{\theECLRHSecondLine}\\[-4pt]
  \rlap{\VRHDW{0.5pt}{0pt}{\textwidth}}&\\
  \end{tabular*}}}

\ECRRHFirstLine{\relax}% default
\ECRRHSecondLine{\fs.7.9.{\rm \theECTYPE}{\bf\theECRUNAUTHOR\theECAUpunct}{\it\theECRUNTITLE}}% default
\ECLRHFirstLine{\relax}% default
\ECLRHSecondLine{\fs.7.9.{\rm \theECTYPE}{\bf\theECRUNAUTHOR\theECAUpunct}{\it\theECRUNTITLE}}% default


\if@BLINDREV
\RRHFirstLine{\bf Authors' names blinded for peer review}% default
\RRHSecondLine{\fs.7.9.\rm Article submitted to {\it\theJOURNAL}; manuscript no. {\theMANUSCRIPTNO}}% default
\LRHFirstLine{\bf Authors' names blinded for peer review}% default
\LRHSecondLine{\fs.7.9.\rm Article submitted to {\it\theJOURNAL}; manuscript no. {\theMANUSCRIPTNO}}% default
\fi

\if@NONBLINDREV
\RRHFirstLine{\bf\theRUNAUTHOR:\enskip {\it\theRUNTITLE}}% default
\RRHSecondLine{\fs.7.9.\rm Article submitted to {\it\theJOURNAL}; manuscript no. {\theMANUSCRIPTNO}}% default
\LRHFirstLine{\bf\theRUNAUTHOR:\enskip {\it\theRUNTITLE}}% default
\LRHSecondLine{\fs.7.9.\rm Article submitted to {\it\theJOURNAL}; manuscript no. {\theMANUSCRIPTNO}}% default
\fi

\let\savesetoddRF=\setoddRF
\let\savesetevenRF=\setevenRF
\let\savesetoddRH=\setoddRH
\let\savesetevenRH=\setevenRH

%%\def\ThePage{\thepage}%

\def\ps@headings{%
    \def\@oddfoot{\setoddRF}%
    \def\@evenfoot{\setevenRF}%
    \def\@oddhead{\CROPMARKS\setoddRH}%
    \def\@evenhead{\CROPMARKS\setevenRH}%
    \let\@mkboth\markboth}

\def\ps@ECheadings{%
    \def\@oddfoot{\relax}%
    \def\@evenfoot{\relax}%
    \def\@oddhead{\CROPMARKS\setoddECRH}%
    \def\@evenhead{\CROPMARKS\setevenECRH}%
    \let\@mkboth\markboth}

%----- first page

\def\setfirstoddFOOT{%
  \raisebox{-24pt}[0pt][0pt]{\hbox to \textwidth{\hfill\fs.8.8.\thepage\hfill}}%
  \global\titlefalse}%

\def\setfirstevenFOOT{%
  \raisebox{-24pt}[0pt][0pt]{\hbox to \textwidth{\hfill\fs.8.8.\thepage\hfill}}%
  \global\titlefalse}%

\def\ps@firstpage{%
  \iftitle\global\titlefalse\let\@mkboth\markboth
  \def\@oddfoot{\setfirstoddFOOT}%
  \def\@evenfoot{\setfirstevenFOOT}%
  \def\@evenhead{\CROPMARKS\hfil}%
  \def\@oddhead{\CROPMARKS\hfil}%
  \def\sectionmark##1{}%
  \def\subsectionmark##1{}%
  \fi
}%

\def\ARTICLEfirstpage{\global\titletrue\thispagestyle{firstpage}}

\newdimen\adim

\long\def\dropcap#1{\setbox0=\hbox{\fs.24.26.#1\kern1pt}%
  \adim\wd0\hangindent\wd0\hangafter-2\noindent
  \kern-\wd0\smash{\if@COPYEDIT\lower13pt\else\lower10pt\fi\copy0}\relax}

%---- \maketitle and \@maketitle
\def\maketitle{\par
  \begingroup
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
    \def\@makefnmark{{\ifnum\c@footnote=1{*}\else
           \@textsuperscript{{\normalfont\@thefnmark}}\fi}}%
    \long\def\@makefntext##1{\noindent
      \ifnum\c@footnote=1\hbox{*\,}\else
      \hbox{\@textsuperscript{\normalfont\@thefnmark}\,}\fi
      \EGT ##1}%
    \let \footnote \thanks
    \if@twocolumn
      \ifnum \col@number=\@ne
        \@maketitle
      \else
        \twocolumn[\@maketitle]%
      \fi
    \else
      \newpage
      \global\@topnum\z@   % Prevents figures from going at top of page.
      \@maketitle
    \fi
  \@thanks
  \endgroup
  \setcounter{footnote}{0}%
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \global\let\maketitle\relax\global\let\@maketitle\relax\parindent1em\normalsize}

\def\@maketitle{%
  \newpage
  \theARTICLETOP
  \theARTICLETITLE
  \theARTICLEAUTHORS
  \theARTICLEABSTRACT
  \theARTICLERULE
}

%%%%%%%%%%%% first page details
\def\TITLEfont{\rm}% default
\def\AUTHORfont{\rm}% default
\def\AFFfont{\rm}% default

\newdimen\ABSwidth
\ABSwidth=\textwidth \advance\ABSwidth-3pc
\def\ABSfont{\small}% default

%% journal-dependent
\def\TITLEfont{\fs.20.24.\rm}% default
\def\AUTHORfont{\fs.11.13.\rm}% default
\def\AFFfont{\fs.8.10.\rm}% default

\def\theARTICLETITLE{%
  \HOOKtop
  \begin{Center}
  \vspace*{0pt}%
  \TITLEfont\HD{24}{0}\theTITLE\HD{0}{15}%
  \end{Center}}

\def\EMAIL#1{#1}% use within AFF
\def\URL#1{#1}% use within AFF
%\def\EMAIL#1{\href{mailto:#1}{#1}}% when hyperref is used
%\def\URL#1{\href{#1}{#1}}         % when hyperref is used

\def\AUTHOR#1{%
  \begin{Center}
  \AUTHORfont\HD{15}{0}#1\HD{0}{6}\relax
  \end{Center}}
\def\AFF#1{%
  \begin{Center}
  \AFFfont{#1}\relax
  \vskip1.6pt
  \end{Center}}

\def\ARTICLERULE#1{\gdef\theARTICLERULE{#1}}%
% default is to have a rule
\def\theARTICLERULE{%
  \begin{Center}
  \vspace*{12pt}
  \VRHDW{1pt}{0pt}{\textwidth}
  \vspace*{4pt}
  \HOOKc
  \end{Center}}

\def\ACKname#1{\gdef\theACKname{#1}}\def\theACKname{Acknowledgments}%

\if@BIGACK
\long\def\ACKNOWLEDGMENT#1{\vskip12pt plus 3pt minus 2pt
  \noindent{\TEN\bf\theACKname}\endgraf\noindent{\TEN #1\endgraf}\endgraf}
\else
\long\def\ACKNOWLEDGMENT#1{\vskip12pt plus 3pt minus 2pt
  \noindent{\fs.13.15.\bf\theACKname}\endgraf\noindent{\NIN #1\endgraf}\endgraf}
\fi

\if@BLINDREV
\long\def\ACKNOWLEDGMENT#1{}%
\fi

\@BIGACKfalse

\if@MOOR
\long\def\ACKNOWLEDGMENT#1{\section*{\bf\theACKname.}{#1\endgraf}\endgraf}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% -b-VARIOUS-TOOLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%-b-dcolumn
%%%%%%%%%% dcolumn.sty - first original then modified
%% File: dcolumn.dtx Copyright (C) 1992-1996 David Carlisle
%\NeedsTeXFormat{LaTeX2e}
%\ProvidesPackage{dcolumn}
%          [1996/02/28 v1.03 decimal alignment package (DPC)]
%%%\RequirePackage{array}
\def\sfdc{\SFrm}
\def\DC@#1#2#3{%
  \uccode`\~=`#1\relax
  \m@th
  \afterassignment\DC@x\count@#3\relax{#1}{#2}}
\def\DC@x#1\relax#2#3{%
  \ifnum\z@>\count@
    \expandafter\DC@centre
  \else
    \expandafter\DC@right
  \fi
  {#2}{#3}{#1}}
\def\DC@centre#1#2#3{%
  \let\DC@end\DC@endcentre
  \uppercase{\def~}{$\egroup\setbox\tw@=\hbox\bgroup$\sfdc{#2}}%
  \setbox\tw@=\hbox{${\phantom{\sfdc{#2}}}$}%
  \setbox\z@=\hbox\bgroup$\sfdc\mathcode`#1="8000 }
\def\DC@endcentre{$\egroup
    \ifdim \wd\z@>\wd\tw@
      \setbox\tw@=\hbox to\wd\z@{\unhbox\tw@\hfill}%
    \else
      \setbox\z@=\hbox to\wd\tw@{\hfill\unhbox\z@}\fi
    \box\z@\box\tw@}
\def\DC@right#1#2#3{%
  \ifx\relax#3\relax
    \hfill
    \let\DC@rl\bgroup
  \else
    \edef\DC@rl{to\the\count@\dimen@ii\bgroup\hss}%
    \count@\@gobble#3\relax
  \fi
  \let\DC@end\DC@endright
  \uppercase{\def~}{$\egroup\setbox\tw@\hbox to\dimen@\bgroup$\sfdc{#2}}%
   \setbox\z@\hbox{$\sfdc 1$}\dimen@ii\wd\z@
   \dimen@\count@\dimen@ii
   \setbox\z@\hbox{$\sfdc{#2}$}\advance\dimen@\wd\z@
   \setbox\tw@\hbox to\dimen@{}%
   \setbox\z@\hbox\DC@rl$\sfdc\mathcode`#1="8000 }
\def\DC@endright{$\hfil\egroup\box\z@\box\tw@}
\def\DC@endright{$\egroup\box\z@\box\tw@}
\newcolumntype{D}[3]{>{\DC@{#1}{#2}{#3}}c<{\DC@end}}
%
% modified version
%
\def\DCFF@#1#2#3#4{%
  \let\sfdc=#4%
  \uccode`\~=`#1\relax
  \m@th
  \afterassignment\DCFF@x\count@#3\relax{#1}{#2}}
\def\DCFF@x#1\relax#2#3{%
  \ifnum\z@>\count@
    \expandafter\DCFF@centre
  \else
    \expandafter\DCFF@right
  \fi
  {#2}{#3}{#1}}
\def\DCFF@centre#1#2#3{%
  \let\DCFF@end\DCFF@endcentre
  \uppercase{\def~}{$\egroup\setbox\tw@=\hbox\bgroup$\sfdc{#2}}%
  \setbox\tw@=\hbox{${\phantom{\sfdc{#2}}}$}%
  \setbox\z@=\hbox\bgroup$\sfdc\mathcode`#1="8000 }
\def\DCFF@endcentre{$\egroup
    \ifdim \wd\z@>\wd\tw@
      \setbox\tw@=\hbox to\wd\z@{\unhbox\tw@\hfill}%
    \else
      \setbox\z@=\hbox to\wd\tw@{\hfill\unhbox\z@}\fi
    \box\z@\box\tw@}
\def\DCFF@right#1#2#3{%
  \ifx\relax#3\relax
    \hfill
    \let\DCFF@rl\bgroup
  \else
    \edef\DCFF@rl{to\the\count@\dimen@ii\bgroup\hss}%
    \count@\@gobble#3\relax
  \fi
  \let\DCFF@end\DCFF@endright
  \uppercase{\def~}{$\egroup\setbox\tw@\hbox to\dimen@\bgroup$\sfdc{#2}}%
   \setbox\z@\hbox{$\sfdc 1$}\dimen@ii\wd\z@
   \dimen@\count@\dimen@ii
   \setbox\z@\hbox{$\sfdc{#2}$}\advance\dimen@\wd\z@
   \setbox\tw@\hbox to\dimen@{}%
   \setbox\z@\hbox\DCFF@rl$\sfdc\mathcode`#1="8000 }
\def\DCFF@endright{$\hfil\egroup\box\z@\box\tw@}
\def\DCFF@endright{$\egroup\box\z@\box\tw@}
\newcolumntype{F}[4]{>{\DCFF@{#1}{#2}{#3}{#4}}c<{\DCFF@end}}

\newcolumntype{d}[1]{D{.}{.}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%-e-dcolumn

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%-b-Extended \cline
%% \Cline takes 4 arguments
%% #1 = from col.; #2 = to col.; #3 = kern on the left; #4 = kern on the right
%%%%%%%%%%%%%%%%%%%%% MODIFICATION:
\newdimen \clineHT
\newdimen \clineDP
\def\Cline#1#2#3#4{\omit\@multicnt#1\advance\@multispan\m@ne
  \ifnum\@multicnt=\@ne\@firstofone{&\omit}\fi\@multicnt#2%
  \advance\@multicnt-#1\advance\@multispan\@ne
  \hskip#3{\leaders\hrule\@height\arrayrulewidth\hfill}\hskip#4\cr
  \noalign{\vskip-\arrayrulewidth}}
%% \Clinev has #5 for additional vertical skip after it is done
\def\Clinev#1#2#3#4#5{\omit\@multicnt#1%
  \advance\@multispan\m@ne\ifnum\@multicnt=\@ne\@firstofone{&\omit}\fi
  \@multicnt#2\advance\@multicnt-#1\advance\@multispan\@ne
  \hskip#3{\leaders\hrule\@height\arrayrulewidth\hfill}\hskip#4\cr
  \noalign{\vskip-\arrayrulewidth\vskip #5}}
%% \ClineVV has #5 for vertical offset of the cline (plus is down)
\def\ClineVV#1#2#3#4#5{%
  \noalign{\vskip #5}%
  \omit\@multicnt#1%
  \advance\@multispan\m@ne\ifnum\@multicnt=\@ne\@firstofone{&\omit}\fi
  \@multicnt#2\advance\@multicnt-#1\advance\@multispan\@ne
  \hskip#3{\leaders \hrule\@height\arrayrulewidth \hfill}\hskip#4\cr
  \noalign{\vskip-#5\vskip-\arrayrulewidth}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%-e-Extended \cline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% -e-VARIOUS-TOOLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%-e-04set01.sty
%%%\endinput
%%%=============================================================================

%--------------------------------------------------------
\def\Trivlist{\parskip0pt\topsep=0pt\parsep0pt\partopsep0pt\@nmbrlistfalse
  \@trivlist \labelwidth\z@ \leftmargin\z@
  \itemindent\z@ \def\makelabel##1{##1}}

\def\endTrivlist{\if@newlist\@noitemerr\fi
   \if@inlabel\indent\fi
   \ifhmode\unskip \par\fi
   \if@noparlist \else
      \ifdim\lastskip >\z@ \@tempskipa\lastskip \vskip -\lastskip
         \advance\@tempskipa\parskip \advance\@tempskipa -\@outerparskip
         \vskip\@tempskipa
   \fi\@endparenv\fi}
%--------------------------------------------------------

%%% Undoing the general version
\def\thebibliography{}
\def\endthebibliography{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% New numeric bibliography environment (works with \cite) (no NATBIB)
\renewenvironment{thebibliography}[1]
    {\subsection*{\hspace*{0pt}References}%
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\fs.9.10.\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \labelsep5pt
            \advance\leftmargin\labelsep
            \itemsep 2pt plus 2pt minus 0.5pt
            %%\@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \def\newblock{\relax}%
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% For NATBIB use
\def\NatBibNumeric{%
 \renewenvironment{thebibliography}[1]{%
  \bibsection\parindent \z@\bibpreamble\bibfont\list
   {\@biblabel{\arabic{NAT@ctr}}}{%
   \setlength{\labelsep}{5pt}\@bibsetup{##1}\setcounter{NAT@ctr}{0}}%
    \renewcommand\newblock{\hskip .11em \@plus.33em \@minus.07em}%
    \sloppy\clubpenalty4000\widowpenalty4000
    \sfcode`\.=1000\relax
    \let\citeN\cite \let\shortcite\cite
    \let\citeasnoun\cite
 }{\def\@noitemerr{%
  \PackageWarning{natbib}
     {Empty `thebibliography' environment}}%
  \endlist\vskip-\lastskip}%
}

\if@MOOR
\def\NatBibNumeric{%
 \renewenvironment{thebibliography}[1]{%
  \section*{\hspace*{-10pt}References}\parindent \z@\bibpreamble\bibfont\list
   {\@biblabel{\arabic{NAT@ctr}}}{%
   \setlength{\labelsep}{5pt}\@bibsetup{##1}\setcounter{NAT@ctr}{0}}%
    \renewcommand\newblock{\hskip .11em \@plus.33em \@minus.07em}%
    \sloppy\clubpenalty4000\widowpenalty4000
    \sfcode`\.=1000\relax
    \let\citeN\cite \let\shortcite\cite
    \let\citeasnoun\cite
 }{\def\@noitemerr{%
  \PackageWarning{natbib}
     {Empty `thebibliography' environment}}%
  \endlist\vskip-\lastskip}%
}%
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%--------------------------------------------------------

\def\mcr{\\[-.6em] \\ }
\newenvironment{pMatrix}[1]{\bgroup\arraycolsep.5em
  \left(\kern-.2em\begin{array}{#1}}{\end{array}\kern-.2em\right)\egroup}
\newenvironment{bMatrix}[1]{\bgroup\arraycolsep.5em
  \left[\kern-.2em\begin{array}{#1}}{\end{array}\kern-.2em\right]\egroup}
\newenvironment{vMatrix}[1]{\bgroup\arraycolsep.5em
  \left|\kern-.2em\begin{array}{#1}}{\end{array}\kern-.2em\right|\egroup}
\newenvironment{Matrix}[1]{\bgroup\arraycolsep.5em
  \begin{array}{#1}}{\end{array}\egroup}
\newenvironment{Array}[1]{\bgroup\arraycolsep0.139em
  \begin{array}{#1}}{\end{array}\egroup}

%--------------------------------------------------------

\def\up{\HD{13}{0}}% for tables
\def\down{\HD{0}{5}}%


\skip\footins=12pt plus 8.1pt minus 5pt
%
\def\EquationsNumberedThrough{%
\def\theequation{\arabic{equation}}%
\def\ECEquationsNumberedThrough{%
\setcounter{equation}{0}\let\oldtheequation=\theequation\def\theequation{EC.\oldtheequation}%
}%
\def\ECHowEquations{\ECEquationsNumberedThrough}%
}
%
\def\EquationsNumberedBySection{%
\@addtoreset{equation}{section}%
\def\theequation{\thesection.\arabic{equation}}%
\def\ECEquationsNumberedBySection{%
\setcounter{equation}{0}\let\oldtheequation=\theequation\def\theequation{EC.\oldtheequation}%
}%
\def\ECHowEquations{\ECEquationsNumberedBySection}%
}
%
\EquationsNumberedThrough % default: 1, 2, 3,

\arraycolsep 1.8pt
\tabcolsep 4pt
\arrayrulewidth .4pt
\doublerulesep 2pt
\tabbingsep\labelsep

%--------------------------------------------------------

%%%=============================================================================
%%% LISTS %%
\newdimen\labelwidthi
\newdimen\labelwidthii
\newdimen\labelwidthiii
\newdimen\labelwidthiv
\def\normal@labelsep{0.5em}
\labelsep\normal@labelsep
\settowidth{\labelwidthi}{\rm(iii)}
\settowidth{\labelwidthii}{\rm(d)}
\settowidth{\labelwidthiii}{\rm(iii)}
\settowidth{\labelwidthiv}{\rm(M)}
\leftmargini\labelwidthi    \advance\leftmargini\labelsep
\leftmarginii\labelwidthii  \advance\leftmarginii\labelsep
\leftmarginiii\labelwidthiii \advance\leftmarginiii\labelsep
\leftmarginiv\labelwidthiv  \advance\leftmarginiv\labelsep
\def\setleftmargin#1#2{\settowidth{\@tempdima}{#2}\labelsep\normal@labelsep
  \csname labelwidth#1\endcsname\@tempdima
  \@tempdimb\@tempdima \advance\@tempdimb\labelsep
  \csname leftmargin#1\endcsname\@tempdimb}
\def\@listI{\leftmargin\leftmargini
  \labelwidth\labelwidthi \labelsep\normal@labelsep
  \topsep \z@ \partopsep\z@ \parsep\z@ \itemsep\z@
  \listparindent 1em}
\def\@listii{\leftmargin\leftmarginii
  \labelwidth\labelwidthii \labelsep\normal@labelsep
  \topsep\z@ \partopsep\z@ \parsep\z@ \itemsep\z@
  \listparindent 1em}
\def\@listiii{\leftmargin\leftmarginiii
  \labelwidth\labelwidthiii \labelsep\normal@labelsep
  \topsep\z@ \partopsep\z@ \parsep\z@ \itemsep\z@
  \listparindent 1em}
\def\@listiv{\leftmargin\leftmarginiv
  \labelwidth\labelwidthiv \labelsep\normal@labelsep
  \topsep\z@ \partopsep\z@ \parsep\z@ \itemsep\z@
  \listparindent 1em}
\let\@listi\@listI
\@listi
\def\left@label#1{{#1}\hss}
\def\right@label#1{\hss\llap{#1}}
\def\thick@label#1{\hspace\labelsep #1}
\newcount\@maxlistdepth
\@maxlistdepth=4
%
\setlength  \labelsep  {.5em}
\setlength  \labelwidth{\leftmargini}
\addtolength\labelwidth{-\labelsep}
\@beginparpenalty -\@lowpenalty
\@endparpenalty   -\@lowpenalty
\@itempenalty     -\@lowpenalty
\def\labelitemi{$\bullet$}          \def\labelitemii{$\cdot$}
\def\labelenumi{(\theenumi)}        \def\theenumi{\arabic{enumi}}
\def\labelenumii{(\alph{enumii})}   \def\theenumii{\theenumi\alph{enumii}}
\def\labelenumiii{(\roman{enumiii})}\def\theenumiii{\theenumii.\roman{enumiii}}
\def\labelenumiv{(\Alph{enumiv})}   \def\theenumiv{\theenumiii.\Alph{enumiv}}
\def\OLDenumerate{%
  \ifnum \@enumdepth >\@maxlistdepth
    \@toodeep
  \else
    \advance\@enumdepth \@ne
    \edef\@enumctr{enum\romannumeral\the\@enumdepth}%
    \list{\csname label\@enumctr\endcsname}%
       {\usecounter{\@enumctr}
    \leftmargin16pt
       \let\makelabel=\right@label}
  \fi}
\def\OLDitemize{%
  \ifnum \@itemdepth >\@maxlistdepth
    \@toodeep
  \else
    \advance\@itemdepth \@ne
    \edef\@itemitem{labelitem\romannumeral\the\@itemdepth}%
     \setleftmargin{i}{--}%
     \setleftmargin{ii}{$\cdot$}%
    \list{\csname\@itemitem\endcsname}%
       {\let\makelabel\right@label}
  \fi}
\def\verse{\let\\=\@centercr
  \list{}{\itemsep\z@
  \itemindent \z@
  \listparindent\z@
  \rightmargin 1em
  \leftmargin \rightmargin}\item[]}
\let\endverse\endlist
\def\quotation{\list{}{\itemindent\z@
 \leftmargin 1em \rightmargin 1em
  \parsep \z@ }\item[]}
\let\endquotation=\endlist
\def\quote{\list{}{\itemindent\z@
   \leftmargin 1em \rightmargin 1em}%
\item[]}
\let\endquote=\endlist
\def\descriptionlabel#1{\hspace\labelsep \itshape #1}
\def\description{\list{}{\labelwidth\z@
  \leftmargin \z@ \itemindent \z@ %-\leftmargin
  \let\makelabel\descriptionlabel}}
\let\enddescription\endlist
%%%%%%%%%%%%%%-e-04listcl.sty
%%%\endinput
%%%%%%%%%%%%%% -b-newlst1 (enumerate, henumerate, ...)
\def\labelitemi{{\makebox[0.5em][s]{\hss\textbullet\hss}}}
\def\labelitemii{{\makebox{\normalfont---\hspace*{-0.35em}}}}
\def\labelitemiii{{\makebox{\normalfont\textasteriskcentered}}}
\def\labelitemiv{{\makebox{\normalfont\textperiodcentered}}}

\renewcommand\theenumi{\@arabic\c@enumi}
\renewcommand\theenumii{\@alph\c@enumii}
\renewcommand\theenumiii{\@roman\c@enumiii}
\renewcommand\theenumiv{\@Alph\c@enumiv}
\renewcommand\labelenumi{{\rm\theenumi.}}
\renewcommand\labelenumii{{\rm(\theenumii)}}
\renewcommand\labelenumiii{{\rm\theenumiii.}}
\renewcommand\labelenumiv{{\rm\theenumiv.}}
\renewcommand\p@enumii{\theenumi}
\renewcommand\p@enumiii{\theenumi(\theenumii)}
\renewcommand\p@enumiv{\p@enumiii\theenumiii}

\newcommand*\descrlabel[1]{\hspace\labelsep\normalfont #1}

%=====================================================================
\def\descr{%
  \ifnum \@itemdepth >\thr@@\@toodeep\else
    \advance\@itemdepth\@ne
    \list{}
    {\DescrListParams}%
  \fi}

\def\DescrListParams{%
\leftmargin\z@ \labelwidth\z@
\ifnum \@itemdepth=1\itemindent1em
\else  \ifnum \@itemdepth=2\itemindent2em
\else \itemindent\labelsep\advance\itemindent3em \fi\fi
\let\makelabel\descrlabel}

\let\enddescr=\endlist
%=====================================================================

\def\hdescr{%
  \ifnum \@itemdepth >\thr@@\@toodeep\else
    \advance\@itemdepth\@ne
    \list{}
    {\HDescrListParams}%
  \fi}

\def\HDescrListParams{%
\leftmargin\z@ \parsep\z@ \itemsep\z@ \parskip\z@ \topsep\z@ \partopsep\z@ \labelsep0.5em \labelwidth\z@
\ifnum \@itemdepth=1 \leftmargin1em \itemindent-1em
\else \ifnum \@itemdepth=2 \leftmargin1em \itemindent-1em
\else \leftmargin1em \itemindent-1em \fi\fi
\let\makelabel\descrlabel}

\let\endhdescr=\endlist
%=====================================================================

\def\enumerate{%
  \ifnum \@enumdepth >\thr@@\@toodeep\else
    \advance\@enumdepth\@ne
    \edef\@enumctr{enum\romannumeral\the\@enumdepth}%
      \expandafter
      \list
        \csname label\@enumctr\endcsname
        {\EnumListParams}%
  \fi}

\def\EnumListParams{%
\usecounter\@enumctr%
\leftmargin\z@ \parsep\z@ \itemsep\z@ \parskip\z@ \topsep\z@ \partopsep\z@ \labelsep0.5em \labelwidth\z@
\ifnum \@enumdepth=1\itemindent=1.5em
\else  \ifnum \@enumdepth=2\itemindent=2.777em
\else  \ifnum \@enumdepth=3\itemindent=3.777em
\else  \itemindent=4.277em \fi\fi\fi
\def\makelabel##1{{##1}}}

\let\endenumerate =\endlist
%=====================================================================

\def\enumitemize{%
  \ifnum \@enumdepth >\thr@@\@toodeep\else
    \advance\@enumdepth\@ne
    \edef\@enumctr{enum\romannumeral\the\@enumdepth}%
      \expandafter
      \list
        {\makebox[0.5em][s]{\hss\textbullet\hss}}%\csname label\@enumctr\endcsname
        {\EnumitemizeListParams}%
  \fi}

\def\EnumitemizeListParams{%
\usecounter\@enumctr%
\leftmargin\z@ \parsep\z@ \itemsep\z@ \parskip\z@ \topsep\z@ \partopsep\z@ \labelsep0.5em \labelwidth\z@
\ifnum \@enumdepth=1\itemindent=1.5em
\else  \ifnum \@enumdepth=2\itemindent=2.777em
\else  \ifnum \@enumdepth=3\itemindent=3.777em
\else  \itemindent=4.277em \fi\fi\fi
\def\makelabel##1{{##1}}}

\let\endenumitemize =\endlist
%=====================================================================

\def\henumerate{%
  \ifnum \@enumdepth >\thr@@\@toodeep\else
    \advance\@enumdepth\@ne
    \edef\@enumctr{enum\romannumeral\the\@enumdepth}%
      \expandafter
      \list
        \csname label\@enumctr\endcsname
        {\HenumListParams}%
  \fi}

\def\HenumListParams{%
\usecounter\@enumctr%
\leftmargin\z@ \parsep\z@ \itemsep\z@ \parskip\z@ \topsep\z@ \partopsep\z@ \labelsep0.5em
\ifnum \@enumdepth=1\leftmargin=1.277em
\else  \ifnum \@enumdepth=2\leftmargin=1.8em
\else  \ifnum \@enumdepth=3\leftmargin=1.65em
\else  \leftmargin=1.55em\fi\fi\fi
\def\makelabel##1{\hss\llap{##1}}}

\let\endhenumerate=\endlist
%=====================================================================

\def\itemize{%
  \ifnum \@itemdepth >\thr@@\@toodeep\else
    \advance\@itemdepth\@ne
    \edef\@itemitem{labelitem\romannumeral\the\@itemdepth}%
    \expandafter
    \list
      \csname\@itemitem\endcsname
      {\ItemizeListParams}%
  \fi}

\def\ItemizeListParams{%
\leftmargin\z@ \parsep0\z@ \itemsep\z@ \parskip\z@ \topsep\z@ \partopsep\z@ \labelsep0.5em \labelwidth\z@
\ifnum \@itemdepth=1 \itemindent1.5em
\else \ifnum \@itemdepth=2 \itemindent2.5em
\else \ifnum \@itemdepth=3 \itemindent3.5em
\else \itemindent4.5em \fi\fi\fi
\def\makelabel##1{{##1}}}

\let\enditemize =\endlist
%=====================================================================

\def\hitemize{%
  \ifnum \@itemdepth >\thr@@\@toodeep\else
    \advance\@itemdepth\@ne
    \edef\@itemitem{labelitem\romannumeral\the\@itemdepth}%
    \expandafter
    \list
      \csname\@itemitem\endcsname
      {\HitemizeListParams}%
  \fi}

\def\HitemizeListParams{%
\leftmargin\z@ \parsep\z@ \itemsep\z@ \parskip\z@ \topsep\z@ \partopsep\z@ \labelsep0.5em \labelwidth\z@
\ifnum \@itemdepth=1 \leftmargin 1em \itemindent-0.5em
\else \ifnum \@itemdepth=2 \leftmargin1.15em \itemindent-0.65em
\else \ifnum \@itemdepth=3 \leftmargin1em \itemindent -0.5em
\else \leftmargin1em \itemindent-0.5em \fi\fi\fi
\def\makelabel##1{{##1}}}

\let\endhitemize =\endlist
%=====================================================================
%%% -e-newlst1
%%%=============================================================================


%%%\input{04thmo01.sty}% theorems
%%%=============================================================================
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%-b-04thmo01.sty (derived from THEOREM for MOOR)
%%%\RequirePackage{theorem}

\gdef\th@TH{%
  \def\theorem@headerfont{\normalfont\TheoremHeaderFont}%
  \theorempreskipamount=6pt plus 3pt minus 2pt \theorempostskipamount=6pt plus 3pt minus 2pt
  \if@MOOR\labelsep1em\else\labelsep0.5em\fi
  \def\@begintheorem##1##2{\normalfont\TheoremTextFont
        \item[\if@OPRE\else\hspace*{1em}\fi\hskip\labelsep
          \theorem@headerfont ##1\ ##2.]}%
  \def\@opargbegintheorem##1##2##3{\normalfont\TheoremTextFont
        \item[\if@OPRE\else\hspace*{1em}\fi\hskip\labelsep
          \theorem@headerfont ##1\ ##2\ {\bf(##3)}.]}}

\gdef\th@THkey{%
  \def\theorem@headerfont{\normalfont\TheoremHeaderFont}%
  \theorempreskipamount=6pt plus 3pt minus 2pt \theorempostskipamount=6pt plus 3pt minus 2pt
  \if@MOOR\labelsep1em\else\labelsep0.5em\fi
  \def\@begintheorem##1##2{\normalfont\TheoremTextFont
        \item[\if@OPRE\else\hspace*{1em}\fi\hskip\labelsep
          \theorem@headerfont ##1\ ##2.]}%
  \def\@opargbegintheorem##1##2##3{\normalfont\TheoremTextFont
        \item[\if@OPRE\else\hspace*{1em}\fi\hskip\labelsep
          \theorem@headerfont {##3}]}}

\gdef\th@EX{%
  \def\theorem@headerfont{\normalfont\ExampleHeaderFont}%
  \if@OPRE
  \theorempreskipamount=6pt plus 3pt minus 2pt \theorempostskipamount=6pt plus 3pt minus 2pt
  \else
  \theorempreskipamount=0pt\theorempostskipamount=0pt
  \fi
  \if@MOOR\labelsep1em\else\labelsep0.5em\fi
  \def\@begintheorem##1##2{\normalfont\ExampleTextFont
        \item[\if@OPRE\else\hspace*{1em}\fi\hskip\labelsep \theorem@headerfont ##1\ ##2.]}%
  \def\@opargbegintheorem##1##2##3{\normalfont\ExampleTextFont
        \item[\if@OPRE\else\hspace*{1em}\fi\hskip\labelsep \theorem@headerfont ##1\ ##2\ {(##3)}.]}}

\gdef\th@EXkey{%
  \def\theorem@headerfont{\normalfont\ExampleHeaderFont}%
  \if@OPRE
  \theorempreskipamount=6pt plus 3pt minus 2pt \theorempostskipamount=6pt plus 3pt minus 2pt
  \else
  \theorempreskipamount=0pt\theorempostskipamount=0pt
  \fi
  \if@MOOR\labelsep1em\else\labelsep0.5em\fi
  \def\@begintheorem##1##2{\normalfont\ExampleTextFont
        \item[\if@OPRE\else\hspace*{1em}\fi\hskip\labelsep \theorem@headerfont ##1\ ##2.]}%
  \def\@opargbegintheorem##1##2##3{\normalfont\ExampleTextFont
        \item[\if@OPRE\else\hspace*{1em}\fi\hskip\labelsep \theorem@headerfont {##3}]}}

\def\TheoremHeaderFont{\mdseries\scshape}
\def\TheoremTextFont{\thit}
\def\ExampleHeaderFont{\mdseries\scshape}
\def\ExampleTextFont{\rm}

%% Use for proper proofs that end with extra space (regardless of the use
%% or non-use of \qed (=the black box)
\def\proof#1{\Trivlist\item[\hspace*{1em}\hskip\labelsep{\it #1\enskip }]\ignorespaces}
\def\endproof{\endTrivlist\addvspace{0pt}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%-e-04thmo01.sty
%%%\endinput
%%%=============================================================================

\JOURNAL{}%{Journal Name Option Missing!}

\def\theARTICLETOP{%
  \vspace*{-57pt}
  \begin{Center}
  \parbox[t][60pt][t]{\textwidth}{%
  \theARTICLETOPLEFT\hfill\theARTICLETOPRIGHT}\\[10pt]
  \parbox{36pc}{\fs.10.11.\bf\textcolor{red}{Authors are encouraged to submit new papers to INFORMS journals by means of
a style file template, which includes the journal title. However, use of a
template does not certify that the paper has been accepted for publication
in the named journal. INFORMS journal templates are for the exclusive
purpose of submitting to an INFORMS journal and should not be used to
distribute the papers in print or online or to submit the papers to another
publication.}}
\vspace*{12pt}
  \end{Center}}

% default values
\def\HOOKtop{\vspace*{0pt}}%
\def\HOOKa{\vspace*{0pt}}%
\def\HOOKb{\vspace*{0pt}}%
\def\HOOKc{\vspace*{0pt}}%

\def\MANUSCRIPTNO#1{\gdef\theMANUSCRIPTNO{#1}}%
  \def\theMANUSCRIPTNO{(Please, provide the manuscript number!)}%{Manuscript number}%

%
\long\def\theARTICLETOPLEFT{{\tabcolsep0pt\fs.8.10.%
\begin{tabular}[t]{l}\null\quad\null\\[0pt]
  \fs.10.10.{\bfseries\sffamily\MakeUppercase{\theJOURNAL}}\\[1pt]
  Vol.~\theVOLUME, No.~\theNO, \theMONTH~\theYEAR, \thePAGERANGE\\
  {\sc issn}\,\theISSN\SEPBAR{\sc eissn}\,\theEISSN\SEPBAR
  \theSHORTYEAR\SEPBAR\theISSUE\SEPBAR\theLONGFIRSTPAGE
\end{tabular}}}%
\def\theARTICLETOPRIGHT{{\tabcolsep0pt\fs.8.10.%
\begin{tabular}[t]{r}\null\quad\null\\[0pt]
  {\fs.16.16.\bfseries\sffamily INFORMS}\\[1pt]
  {\sc doi}\,\theDOI\\
  \copyright\,\theYEAR~INFORMS\end{tabular}}}%
%

\if@BLINDREV
%
\long\def\theARTICLETOPLEFT{{\tabcolsep0pt\fs.12.14.\bf
\begin{tabular}{l}\HD{25}{0}Submitted to {\bi\theJOURNAL}\\
manuscript {\theMANUSCRIPTNO}\end{tabular}}}%
\def\theARTICLETOPRIGHT{}%
%
%\def\theHISTORY{}%
\fi

\if@NONBLINDREV
%
\long\def\theARTICLETOPLEFT{{\tabcolsep0pt\fs.12.14.\bf
\begin{tabular}{l}\HD{25}{0}Submitted to {\bi\theJOURNAL}\\
manuscript {\theMANUSCRIPTNO}\end{tabular}}}%
\def\theARTICLETOPRIGHT{}%
%
\fi

\def\ABSfont{\EGT}

\def\theARTICLEABSTRACT{%
  \begin{Center}
  \HOOKb
  \vspace*{18pt}
  \begin{minipage}{\ABSwidth}\parindent1em
    \ABSfont
    \noindent\theABSTRACT\endgraf
    \vskip5pt
    \theKEYWORDS
    \theSUBJECTCLASS
    \theAREAOFREVIEW
    \theMSCCLASS
    \theORMSCLASS
    \if@BLINDREV\else\theHISTORY\fi
  \end{minipage}%
  \vspace*{0pt}
  \end{Center}}

%SSSSSSS

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%\input{04scmo01.sty}
%%%=============================================================================
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%-b-04scmo01.sty (sectioning in MOOR)
\setcounter{secnumdepth}{3}
\newcounter {part}
\newcounter {chapter}
\newcounter {section}
\newcounter {subsection}[section]
\newcounter {subsubsection}[subsection]
\newcounter {paragraph}[subsubsection]
\newcounter {subparagraph}[paragraph]
\renewcommand\thepart         {\@Roman\c@part}
\renewcommand\thesection      {\@arabic\c@section}
\renewcommand\thesubsection   {\thesection.\@arabic\c@subsection}
\renewcommand\thesubsubsection{\thesubsection.\@arabic\c@subsubsection}
\renewcommand\theparagraph    {\thesubsubsection.\@arabic\c@paragraph}
\renewcommand\thesubparagraph {\theparagraph.\@arabic\c@subparagraph}
%-------------------------------------------------
\def\@startsection#1#2#3#4#5#6{%
  \if@noskipsec \leavevmode \fi
  \par
  \@tempskipa #4\relax
  \@afterindenttrue
  \ifdim \@tempskipa <\z@
    \@tempskipa -\@tempskipa \@afterindentfalse
  \fi
  \if@nobreak
    \everypar{}%
  \else
    \addpenalty\@secpenalty\addvspace\@tempskipa
  \fi
  \@ifstar
    {\@ssect{#3}{#4}{#5}{#6}}%
    {\@dblarg{\@sect{#1}{#2}{#3}{#4}{#5}{#6}}}}
%-------------------------------------------------
\def\@sect#1#2#3#4#5#6[#7]#8{%
  \ifnum #2>\c@secnumdepth
    \let\@svsec\@empty
  \else
    \refstepcounter{#1}%
%%%    \protected@edef\@svsec{\@seccntformat{#1}\relax}%
    \protected@edef\@svsec{\ifnum \c@nowappendix=1
       \ifnum#2=1\@appseccntformat{#1}\else\@seccntformat{#1}\fi
       \else\@seccntformat{#1}\fi}%
%%%%%\edef\@svsec{\indent\ifnum \c@nowappendix=1 \ifnum#2=1{Appendix~}\fi\fi
%%%%%     \csname the#1\endcsname \ifnum#2=1.\fi \hskip 5pt }\fi
  \fi
  \@tempskipa #5\relax
  \ifdim \@tempskipa>\z@
    \begingroup
      #6{%
        \@hangfrom{\hskip #3\relax\@svsec}%
          \interlinepenalty \@M #8\@@par}%
    \endgroup
    \csname #1mark\endcsname{#7}%
    \addcontentsline{toc}{#1}{%
      \ifnum #2>\c@secnumdepth \else
        \protect\numberline{\csname the#1\endcsname}%
      \fi
      #7}%
  \else
    \def\@svsechd{%
      #6{\hskip #3\relax
      \@svsec #8}%
      \csname #1mark\endcsname{#7}%
      \addcontentsline{toc}{#1}{%
        \ifnum #2>\c@secnumdepth \else
          \protect\numberline{\csname the#1\endcsname}%
        \fi
        #7}}%
  \fi
  \@xsect{#5}}
%-------------------------------------------------
\def\@xsect#1{%
  \@tempskipa #1\relax
  \ifdim \@tempskipa>\z@
    \par \nobreak
    \vskip \@tempskipa
    \@afterheading
  \else
    \@nobreakfalse
    \global\@noskipsectrue
    \everypar{%
      \if@noskipsec
        \global\@noskipsecfalse
       {\setbox\z@\lastbox}%
        \clubpenalty\@M
        \begingroup \@svsechd \endgroup
        \unskip
        \@tempskipa #1\relax
        \hskip -\@tempskipa
      \else
        \clubpenalty \@clubpenalty
        \everypar{}%
      \fi}%
  \fi
  \ignorespaces}
%-------------------------------------------------
\def\@seccntformat#1{{\upshape\csname the#1\endcsname.}\hskip1.0em }
\def\@appseccntformat#1{{\upshape Appendix~\csname the#1\endcsname:}\hskip1.0em }
\if@OPRE
\def\@seccntformat#1{{\upshape\csname the#1\endcsname.}\enskip }
\def\@appseccntformat#1{{\upshape Appendix~\csname the#1\endcsname:}\enskip }
\fi
\if@MOOR
\def\@seccntformat#1{{\upshape\csname the#1\endcsname.}\enskip }
\def\@appseccntformat#1{{\upshape Appendix~\csname the#1\endcsname:}\enskip }
\fi
%-------------------------------------------------
\def\@ssect#1#2#3#4#5{%
  \@tempskipa #3\relax
  \ifdim \@tempskipa>\z@
    \begingroup
      #4{%
        \@hangfrom{\hskip #1}%
          \interlinepenalty \@M #5\@@par}%
    \endgroup
  \else
    \def\@svsechd{#4{\hskip #1\relax #5}}%
  \fi
  \@xsect{#3}}
%-------------------------------------------------

\def\section{\@startsection{section}{1}{\z@}{-15pt plus -5pt minus -4pt}{0.01pt}%
    {\fs.13.15.\bf\RAGG}}
\def\subsection{\@startsection{subsection}{2}{\z@}{-12pt plus -4pt minus -2pt}{0.01pt}
    {\fs.11.{13.6}.\bf\RAGG}}
\def\subsubsection{\@startsection{subsubsection}{3}{10pt}{6pt plus 3pt minus 2pt}{-5pt}
    {\fs.11.{13.6}.\bf}}
\def\paragraph{\@startsection{paragraph}{4}{10pt}{0.1pt plus 0.1pt minus 0.1pt}{-0.5em}%
    {\fs.11.{13.6}.\it}}
\def\subparagraph{\@startsection{subparagraph}{5}{10pt}{0.1pt plus 0.1pt minus 0.1pt}{-1em}%
    {\fs.11.{13.6}.\it}}

%% EC subtitle (what it really is: Proofs, Technical Appendix, ...)
\def\ECHead#1{\par\noindent{\raggedright\fs.15.18.\bf #1\endgraf}}

%\def\section{\@startsection{section}{1}{0pt}{-12pt plus -9pt minus -4pt}{0.01pt}{\fs.13.15.\bf}}%
%\def\subsection{\@startsection{subsection}{2}{0pt}{-12pt plus -6pt minus -2pt}{3pt}{\fs.12.14.\bf}}%
%\def\subsubsection{\@startsection{subsubsection}{3}{0pt}{6pt plus 5pt minus 1pt}{-1em}{\TEN\bf}}%
%\def\paragraph{\@startsection{paragraph}{4}{1.0em}{-0.01pt}{-1em}{\bi}}%
%\def\subparagraph{\@startsection{subparagraph}{5}{1.0em}{-0.01pt}{-1em}{\it}}%

\if@OPRE
\def\section{\@startsection {section}{1}{\z@}{-13pt plus -6pt minus -3pt}{4pt}%
  {\fs.13.15.\sffamily\bfseries\RAGG}}%
\def\subsection{\@startsection{subsection}{2}{\z@}{-13pt plus -6pt minus -3pt}{4pt}%
  {\TEN\sffamily\bfseries\RAGG}}%
\def\subsubsection{\@startsection{subsubsection}{3}{1.0em}{6pt plus 4pt minus 2pt}{-10pt}%
  {\TEN\bf}}%
\def\paragraph{\@startsection{paragraph}{4}{1em}{0.1pt plus 0.1pt minus 0.1pt}{-0.5em}{\TEN\it}}%
\def\subparagraph{\@startsection{subparagraph}{5}{1em}{0.1pt plus 0.1pt minus 0.1pt}{-1em}{\TEN\it}}%
\fi

\if@MOOR
\def\section{\@startsection{section}{1}{1em}{12pt plus 2pt minus 4pt}{-1em}{\bf}}%
\def\subsection{\@startsection{subsection}{2}{1em}{12pt plus 2pt minus 2pt}{-1em}{\bf}}%
\def\subsubsection{\@startsection{subsubsection}{3}{1em}{12pt plus 2pt minus 2pt}{-1em}{\bf}}%
\def\paragraph{\@startsection{paragraph}{4}{1em}{6pt plus 1pt minus 2pt}{-1em}{\bi}}%
\def\subparagraph{\@startsection{subparagraph}{5}{1em}{-0.01pt}{-1em}{\it}}%
\fi

%---
\def\ECHowSections{%
\setcounter{section}{0}%
\renewcommand\thesection      {EC.\@arabic\c@section}%
\renewcommand\thesubsection   {\thesection.\@arabic\c@subsection}%
\renewcommand\thesubsubsection{\thesubsection.\@arabic\c@subsubsection}%
\renewcommand\theparagraph    {\thesubsubsection.\@arabic\c@paragraph}%
\renewcommand\thesubparagraph {\theparagraph.\@arabic\c@subparagraph}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% FIGURES and TABLES
\newbox\@tempboxa
\newbox\@tempboxb

\def\FigureCaptionFontStyle{\sffamily\bfseries}%
\def\FigureNameFontStyle{\sffamily\bfseries}%
\def\FigureNoteStyle{\EGT\rm}
\def\FigureNoteName{Note.}

\def\TableCaptionFontStyle{\sffamily\bfseries}%
\def\TableNameFontStyle{\sffamily\bfseries}%
%\def\TableFontSize{\EGT}
\def\TableNoteStyle{\EGT\rm}
\def\TableNoteName{Note.}

\def\NOTE#1{\unskip\hspace*{0em}{\it #1\/}\enskip}

\if@OPRE
\def\FigureCaptionFontStyle{\mdseries}%
\def\FigureNameFontStyle{\bfseries}%
\def\TableCaptionFontStyle{\mdseries}%
\def\TableNameFontStyle{\bfseries}%
\def\TableNoteStyle{\EGT\sffamily}
\def\NOTE#1{\unskip\hspace*{0em}{\sffamily\itshape #1\/}\enskip}
\fi

\long\def\@makefigurecaption#1#2{\EGT\FigureCaptionFontStyle
  \setbox9=\hbox{\FigureNameFontStyle #1\kern16pt}\hangindent\wd9\noindent
  \HD{9}{0}\hbox{\FigureNameFontStyle #1\kern16pt}\ignorespaces #2\HD{0}{9}\endgraf}
\long\def\@maketablecaption#1#2{\EGT\TableCaptionFontStyle
  \setbox9=\hbox{\TableNameFontStyle #1\kern16pt}\hangindent\wd9\noindent
  \HD{9}{0}\hbox{\TableNameFontStyle #1\kern16pt}\ignorespaces #2\HD{0}{5}\endgraf}

%% MJ-4/19/2006
\if@MNSC
\long\def\@makefigurecaption#1#2{\EGT\FigureCaptionFontStyle
  \begin{Center}\HD{9}{0}{\FigureNameFontStyle #1\kern16pt}\ignorespaces #2\HD{0}{0}\endgraf\end{Center}}
\fi
\if@IJOC
\long\def\@makefigurecaption#1#2{\EGT\FigureCaptionFontStyle
  \setbox9=\hbox{\FigureNameFontStyle #1\kern16pt}\hangindent\wd9\noindent
  \HD{9}{0}\hbox{\FigureNameFontStyle #1\kern16pt}\ignorespaces #2\HD{0}{0}\endgraf}
\fi
\if@TRSC
\long\def\@makefigurecaption#1#2{\EGT\FigureCaptionFontStyle
  \setbox9=\hbox{\FigureNameFontStyle #1\kern16pt}\hangindent\wd9\noindent
  \HD{9}{0}\hbox{\FigureNameFontStyle #1\kern16pt}\ignorespaces #2\HD{0}{0}\endgraf}
\fi

%% MJ-1/31/2007
\long\def\@maketablecaption#1#2{\EGT\TableCaptionFontStyle
  \begin{Center}\HD{9}{0}{\TableNameFontStyle #1\kern16pt}\ignorespaces #2\HD{0}{5}\endgraf\end{Center}}


\newif\if@rotate \@rotatefalse
\def\rotate{\global\@rotatetrue}
\def\endrotate{\global\@rotatefalse}

%*********************************************
%\if@MNSC

%************************************
\def\FIGURE#1#2#3{%
\long\def\testfignote{#3}%
\long\def\itis@empty{}%
\ifx\testfignote\itis@empty
  \long\def\fignote##1{\relax}%
\else
  \long\def\fignote##1{\par\noindent
  \FigureNoteStyle\HD{11}{0}{\it\FigureNoteName}\enskip ##1\endgraf}%
\fi
\if@rotate
  \setbox4=\hbox to \textheight{\vbox{\hsize\textheight
  \begin{minipage}{\textheight}
  \caption[]{#2}%
  \begin{Center}%
  {#1}%
  \end{Center}%
  \fignote{#3}%
  \end{minipage}}}
\else
  \setbox4=\hbox to \hsize{\vbox{%
  \begin{minipage}{\hsize}
  \caption[]{#2}
  \hbox to\hsize{\hss{#1}\hss}%
  \fignote{#3}%
  \end{minipage}}}
\fi
\if@rotate
  \noindent\vrule width0pt height0.5\textheight depth0.5\textheight
  \hspace*{0.5\textwidth}\rotatebox{90}{\copy4}%
\else
  \box4
\fi}
%************************************
%************************************
\if@IJOC
\def\FIGURE#1#2#3{%
\long\def\testfignote{#3}%
\long\def\itis@empty{}%
\ifx\testfignote\itis@empty
  \long\def\fignote##1{\relax}%
\else
  \long\def\fignote##1{\par\noindent
  \FigureNoteStyle\noindent\HD{11}{0}{\it\FigureNoteName}\enskip ##1\endgraf}%
\fi
\if@rotate
  \setbox4=\hbox to \textheight{\vbox{\hsize\textheight
  \begin{minipage}{\textheight}
  \begin{Center}%
  {#1}%
  \end{Center}%
  \caption[]{#2}%
  \fignote{#3}%
  \end{minipage}}}
\else
  \setbox4=\hbox to \hsize{\vbox{%
  \begin{minipage}{\hsize}
  \hbox to\hsize{\hss{#1}\hss}%
  \caption[]{#2}
  \fignote{#3}%
  \end{minipage}}}
\fi
\if@rotate
  \noindent\vrule width0pt height0.5\textheight depth0.5\textheight
  \hspace*{0.5\textwidth}\rotatebox{90}{\copy4}%
\else
  \box4
\fi}
\fi
%************************************
%************************************
\if@TRSC
\def\FIGURE#1#2#3{%
\long\def\testfignote{#3}%
\long\def\itis@empty{}%
\ifx\testfignote\itis@empty
  \long\def\fignote##1{\relax}%
\else
  \long\def\fignote##1{\par\noindent
  \FigureNoteStyle\noindent\HD{11}{0}{\it\FigureNoteName}\enskip ##1\endgraf}%
\fi
\if@rotate
  \setbox4=\hbox to \textheight{\vbox{\hsize\textheight
  \begin{minipage}{\textheight}
  \begin{Center}%
  {#1}%
  \end{Center}%
  \caption[]{#2}%
  \fignote{#3}%
  \end{minipage}}}
\else
  \setbox4=\hbox to \hsize{\vbox{%
  \begin{minipage}{\hsize}
  \hbox to\hsize{\hss{#1}\hss}%
  \caption[]{#2}
  \fignote{#3}%
  \end{minipage}}}
\fi
\if@rotate
  \noindent\vrule width0pt height0.5\textheight depth0.5\textheight
  \hspace*{0.5\textwidth}\rotatebox{90}{\copy4}%
\else
  \box4
\fi}
\fi
%************************************

\def\TEGT{\TableSpaced}%

% TABLE
\long\def\TABLE#1#2#3{\setbox\tempbox=\hbox{{\TEGT #2}}%
  \tempdim\wd\tempbox\tempdimht\ht\tempbox\advance\tempdimht\dp\tempbox
  \@TABLE{#1}{#2}{#3}{\tempdim}}

\long\def\@TABLE#1#2#3#4{%
\TableSpaced
%\if@COPYEDIT\ifdim\tempdimht<\TableStretchBreak\def\arraystretch{1.5}\else\def\arraystretch{1}\fi\else\fi
\long\def\testtabnote{#3}%
\long\def\itis@empty{}%
\ifx\testtabnote\itis@empty
  \long\def\tabnote##1{\relax}%
\else
  \long\def\tabnote##1{\par\TableNoteStyle\parindent1em\ignorespaces
    \HD{11}{0}##1\endgraf}%
\fi
\if@rotate
  \setbox4=\hbox to \textheight
  {\vbox to \textwidth{\hsize\textheight\vfill\begin{Flushright}% Center
  \begin{minipage}[c]{#4}%
  \caption[]{#1}{\TEGT #2}\tabnote{#3}\end{minipage}
  \end{Flushright}\vfill}}
\else
  \setbox4=\hbox to \hsize{\hss
  \begin{minipage}[t]{#4}%
  \caption[]{#1}{\TEGT #2}\tabnote{#3}\end{minipage}\hss}
\fi
\if@rotate
  \rotatebox{90}{\copy4}%
\else
  \box4
\fi}
%\fi
%*********************
\if@MOOR
\def\FigureCaptionFontStyle{\mdseries}%
\def\TableCaptionFontStyle{\mdseries}%
\long\def\@makefigurecaption#1#2{\EGT
  \FigureCaptionFontStyle
  \setbox\@tempboxa=\hbox{{\sc #1.}\enskip #2}%
  \setbox\@tempboxb=\hbox{#2}%
  \ifdim \wd\@tempboxb < 3pt
    \noindent\null\hfill{\sc #1.}%
    \HD{14}{0}\hfill\null\endgraf
  \else
  \ifdim \wd\@tempboxa >\hsize
    \noindent\hspace*{0em}\HD{14}{0}{\sc #1.}\enskip
    #2\par
  \else
    \noindent\null\hfill{\sc #1.}%
    \enskip #2\HD{14}{0}\hfill\null\endgraf
  \fi\fi}%
\long\def\@maketablecaption#1#2{\EGT
% Set TN followed by the caption see the length
  \setbox\@tempboxa
  \hbox{\TableCaptionFontStyle{\sc #1}.\enskip #2}%
% Set the caption only to examine its existence and length if any
  \setbox\@tempboxb
  \hbox{\TableCaptionFontStyle #2}%
% If no caption, TN centers with no period after it
  \ifdim\wd\@tempboxb < 3pt
    \begin{Center}\TableCaptionFontStyle\HD{8}{0}{\sc #1}\HD{0}{6}\end{Center}
  \else
% If TN+caption shorter than the table
  \ifdim\wd\@tempboxa < \tempdim
    \begin{Center}\TableCaptionFontStyle\HD{8}{0}{\sc #1}.\enskip #2\HD{0}{6}\end{Center}
  \else
% If TN+caption longer than the table
    \noindent\TableCaptionFontStyle\HD{8}{0}{\sc #1}.\enskip #2\HD{0}{6}\endgraf
  \fi\fi}%
%
\def\FIGURE#1#2#3{%
\long\def\testfignote{#3}\long\def\itis@empty{}%
\ifx\testfignote\itis@empty
  \long\def\fignote##1{\relax}%
\else
  \long\def\fignote##1{\par{\FigureNoteStyle
    \parindent1em\HD{10}{0}{\it\FigureNoteName}\enskip
    ##1\HD{0}{3}\vspace*{-3pt}\endgraf}}%
\fi
\if@rotate
  \setbox4=\hbox to \textheight{\vbox{\hsize\textheight
  \begin{minipage}{\textheight}
  \hbox to\hsize{\hss{#1}\hss}%
  \caption[]{#2}
  \fignote{#3}%
  \end{minipage}}}
\else
  \setbox4=\hbox to \hsize{\vbox{%
  \begin{minipage}{\hsize}
  \hbox to\hsize{\hss{#1}\hss}%
  \caption[]{#2}
  \fignote{#3}%
  \end{minipage}}}
\fi
\if@rotate
  \setbox5=\zeroCC{\box4}%
  \par\noindent\hspace*{0.5\textwidth}%
  \vrule width 0pt height 0.5\textheight depth 0.499\textheight
  \rotatebox{90}{\box5}%
\else
  \noindent\box4%
\fi}
%
% TABLE
\def\TABLE#1#2#3{%
  \setbox\tempbox=\hbox{{\TEGT #2}}%
  \tempdim\wd\tempbox\tempdimht\ht\tempbox\advance\tempdimht\dp\tempbox
  \@TABLE{#1}{#2}{#3}{\tempdim}}
%
\def\@TABLE#1#2#3#4{%
%%\if@COPYEDIT\ifdim\tempdimht<\TableStretchBreak\def\arraystretch{1.5}\else\def\arraystretch{1}\fi\else\fi
\TABLESpaced
\long\def\testtabnote{#3}%
\long\def\itis@empty{}%
\ifx\testtabnote\itis@empty
  \long\def\tabnote##1{\relax}%
\else
  \long\def\tabnote##1{\par\TableNoteStyle{\parindent1em
  \HD{13}{0}##1\endgraf}}%
\fi
\if@rotate
  \setbox4=\hbox to #4 %%\textheight
  {\vbox to \textwidth{\hsize #4 %%%\textheight
  \vss
  \begin{minipage}[c]{#4}%
  \caption[]{#1}%
  {\TEGT #2}%
  \tabnote{#3}%
  \end{minipage}%
  \vss}}
\else
  \setbox4=\hbox to \hsize{\hss
  \begin{minipage}[t]{#4}%
  \TEGT
  \caption[]{#1}%
  {\TEGT #2}%
  \tabnote{#3}%
  \end{minipage}\hss}
\fi
\if@rotate
  \setbox5=\zeroCC{\box4}%
  \par\noindent\hspace*{0.5\textwidth}%
  \vrule width 0pt height 0.5\textheight depth 0.499\textheight
  \rotatebox{90}{\box5}%
\else
  \noindent\box4%
\fi}
\fi
%*********************

\def\TheoremsNumberedBySection{%
\theoremstyle{TH}%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{hypothesis}{Hypothesis}[section]
\newtheorem{assumption}{Assumption}[section]
\theoremstyle{EX}
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{problem}{Problem}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{question}{Question}[section]
\newtheorem{answer}{Answer}[section]
\newtheorem{exercise}{Exercise}[section]
%---
\def\ECTheoremsNumberedBySection{%
\setcounter{theorem}{0}\let\oldthetheorem=\thetheorem\def\thetheorem{\oldthetheorem}%
\setcounter{lemma}{0}\let\oldthelemma=\thelemma\def\thelemma{\oldthelemma}%
\setcounter{proposition}{0}\let\oldtheproposition=\theproposition\def\theproposition{\oldtheproposition}%
\setcounter{corollary}{0}\let\oldthecorollary=\thecorollary\def\thecorollary{\oldthecorollary}%
\setcounter{claim}{0}\let\oldtheclaim=\theclaim\def\theclaim{\oldtheclaim}%
\setcounter{conjecture}{0}\let\oldtheconjecture=\theconjecture\def\theconjecture{\oldtheconjecture}%
\setcounter{hypothesis}{0}\let\oldthehypothesis=\thehypothesis\def\thehypothesis{\oldthehypothesis}%
\setcounter{assumption}{0}\let\oldtheassumption=\theassumption\def\theassumption{\oldtheassumption}%
\setcounter{remark}{0}\let\oldtheremark=\theremark\def\theremark{\oldtheremark}%
\setcounter{example}{0}\let\oldtheexample=\theexample\def\theexample{\oldtheexample}%
\setcounter{problem}{0}\let\oldtheproblem=\theproblem\def\theproblem{\oldtheproblem}%
\setcounter{definition}{0}\let\oldthedefinition=\thedefinition\def\thedefinition{\oldthedefinition}%
\setcounter{question}{0}\let\oldthequestion=\thequestion\def\thequestion{\oldthequestion}%
\setcounter{answer}{0}\let\oldtheanswer=\theanswer\def\theanswer{\oldtheanswer}%
\setcounter{exercise}{0}\let\oldtheexercise=\theexercise\def\theexercise{\oldtheexercise}%
}%
\def\ECHowTheorems{\ECTheoremsNumberedBySection}%
%---
}
\def\TheoremsNumberedThrough{%
\theoremstyle{TH}%
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{conjecture}{Conjecture}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{assumption}{Assumption}
\theoremstyle{EX}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{problem}{Problem}
\newtheorem{definition}{Definition}
\newtheorem{question}{Question}
\newtheorem{answer}{Answer}
\newtheorem{exercise}{Exercise}
%---
\def\ECTheoremsNumberedThrough{%
\setcounter{theorem}{0}\let\oldthetheorem=\thetheorem\def\thetheorem{EC.\oldthetheorem}%
\setcounter{lemma}{0}\let\oldthelemma=\thelemma\def\thelemma{EC.\oldthelemma}%
\setcounter{proposition}{0}\let\oldtheproposition=\theproposition\def\theproposition{EC.\oldtheproposition}%
\setcounter{corollary}{0}\let\oldthecorollary=\thecorollary\def\thecorollary{EC.\oldthecorollary}%
\setcounter{claim}{0}\let\oldtheclaim=\theclaim\def\theclaim{EC.\oldtheclaim}%
\setcounter{conjecture}{0}\let\oldtheconjecture=\theconjecture\def\theconjecture{EC.\oldtheconjecture}%
\setcounter{hypothesis}{0}\let\oldthehypothesis=\thehypothesis\def\thehypothesis{EC.\oldthehypothesis}%
\setcounter{assumption}{0}\let\oldtheassumption=\theassumption\def\theassumption{EC.\oldtheassumption}%
\setcounter{remark}{0}\let\oldtheremark=\theremark\def\theremark{EC.\oldtheremark}%
\setcounter{example}{0}\let\oldtheexample=\theexample\def\theexample{EC.\oldtheexample}%
\setcounter{problem}{0}\let\oldtheproblem=\theproblem\def\theproblem{EC.\oldtheproblem}%
\setcounter{definition}{0}\let\oldthedefinition=\thedefinition\def\thedefinition{EC.\oldthedefinition}%
\setcounter{question}{0}\let\oldthequestion=\thequestion\def\thequestion{EC.\oldthequestion}%
\setcounter{answer}{0}\let\oldtheanswer=\theanswer\def\theanswer{EC.\oldtheanswer}%
\setcounter{exercise}{0}\let\oldtheexercise=\theexercise\def\theexercise{EC.\oldtheexercise}%
}%
\def\ECHowTheorems{\ECTheoremsNumberedThrough}%
%---
}
%\TheoremsNumberedThrough% default behavior (in the template): Th. 1, Th. 2, Lemma 1, ...

\def\ECRepeatTheorems{%
\theoremstyle{THkey}%
\newtheorem{repeattheorem}{Theorem}
\newtheorem{repeatlemma}{Lemma}
\newtheorem{repeatproposition}{Proposition}
\newtheorem{repeatcorollary}{Corollary}
\newtheorem{repeatclaim}{Claim}
\newtheorem{repeatconjecture}{Conjecture}
\newtheorem{repeathypothesis}{Hypothesis}
\newtheorem{repeatassumption}{Assumption}
\theoremstyle{EXkey}
\newtheorem{repeatremark}{Remark}
\newtheorem{repeatexample}{Example}
\newtheorem{repeatproblem}{Problem}
\newtheorem{repeatdefinition}{Definition}
\newtheorem{repeatquestion}{Question}
\newtheorem{repeatanswer}{Answer}
\newtheorem{repeatexercise}{Exercise}}


\def\TableStretchBreak{380pt}%

%%%%%%%%%%%%%%%%%%%%%%%%%

\if@DECA
\JOURNAL{Decision Analysis}%
\ISSN{1545-8490}%
\EISSN{1545-8504}%
\fi

\if@IJOC
\JOURNAL{INFORMS Journal on Computing}%
\ISSN{0899-1499}%
\EISSN{1526-5528}%
\OneAndAHalfSpacedXII
\fi

\if@INTE
\JOURNAL{Interfaces}%
\ISSN{0092-2102}%
\EISSN{1526-551X}%
\fi

\if@ISRE
\JOURNAL{Information Systems Research}%
\ISSN{1047-7047}%
\EISSN{1526-5536}%
\fi

\if@MNSC
\JOURNAL{Management Science}%
\ISSN{0025-1909}%
\EISSN{1526-5501}%
\fi

\if@MKSC
\JOURNAL{Marketing Science}%
\ISSN{0732-2399}%
\EISSN{1526-548X}%
\fi

\if@MOOR
\JOURNAL{Mathematics of Operations Research}%
\ISSN{0364-765X}%
\EISSN{1526-5471}%
\fi

\if@MSOM
\JOURNAL{Manufacturing \& Service Operations Management}%
\ISSN{1523-4614}%
\EISSN{1526-5498}%
\fi

\if@OPRE
\JOURNAL{Operations Research}%
\ISSN{0030-364X}%
\EISSN{1526-5463}%
\fi

\if@ORSC
\JOURNAL{Organization Science}%
\ISSN{1047-7039}%
\EISSN{1526-5455}%
\fi

\if@TRSC
\JOURNAL{Transportation Science}%
\ISSN{0041-1655}%
\EISSN{1526-5447}%
\fi

\if@ITED
\JOURNAL{INFORMS Transactions on Education}%
\ISSN{1532-0545}%
\EISSN{1532-0545}%
\fi

\pagestyle{headings}
\pagenumbering{arabic}
\onecolumn\sloppy
\frenchspacing
\flushbottom

\AtBeginDocument{\ARTICLEfirstpage}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%-b-Appendix
%\newcommand\appendix{\par
%  \setcounter{section}{0}%
%  \setcounter{subsection}{0}%
%  \renewcommand\thesection{\@Alph\c@section}}

\def\appendixhead#1{\vskip20pt plus 9pt minus4pt\noindent
  {\AppendixHeadSize\textbf{#1}}\vskip4pt\nobreak}%

\newenvironment{APPENDIX}[1]{\par
  \long\def\testAPP{.\space #1}%
  \long\def\testAPPempty{.\space}%
  \ifx\testAPP\testAPPempty
    \appendixhead{Appendix}%
  \else
    \appendixhead{Appendix. #1}%
  \fi
  \AppendixFontSize
  \def\section{\@startsection{section}{1}{0pt}%
    {-6pt plus -6pt minus -1pt}{2.5pt}{\AppendixSectionHeadSize\bf\RAGG}}
  \def\subsection{\@startsection{subsection}{2}{0pt}%
    {-4pt plus -4pt minus -1pt}{2pt}{\AppendixFontSize\bf\RAGG}}
  \def\subsubsection{\@startsection{subsubsection}{3}{0pt}%
    {3pt plus 3pt minus 1pt}{-1em}{\AppendixFontSize\bf}}
  \if@MOOR
    \def\section{\@startsection{section}{1}{1em}{12pt plus 2pt minus 4pt}{-1em}{\bf}}%
    \def\subsection{\@startsection{subsection}{2}{1em}{12pt plus 2pt minus 2pt}{-1em}{\bf}}%
    \def\subsubsection{\@startsection{subsubsection}{3}{1em}{12pt plus 2pt minus 2pt}{-1em}{\bf}}%
  \fi
  \if@OPRE
    \def\section{\@startsection{section}{1}{0pt}%
      {-6pt plus -6pt minus -1pt}{2.5pt}{\AppendixSectionHeadSize\sffamily\bfseries\RAGG}}
    \def\subsection{\@startsection{subsection}{2}{0pt}%
      {-4pt plus -4pt minus -1pt}{2pt}{\AppendixFontSize\sffamily\bfseries\RAGG}}
    \def\subsubsection{\@startsection{subsubsection}{3}{0pt}%
      {3pt plus 3pt minus 1pt}{-1em}{\AppendixFontSize\bf}}
  \fi
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \setcounter{subsubsection}{0}%
  \renewcommand\thesection{\@Alph\c@section}%
  \parindent1em}
  {\vskip1sp}

\newenvironment{APPENDICES}{%
  \par\setcounter{nowappendix}{1}\relax
  \AppendixFontSize
  \def\section{\@startsection{section}{1}{0pt}%
    {-6pt plus -6pt minus -1pt}{2.5pt}{\AppendixSectionHeadSize\bf\RAGG}}
  \def\subsection{\@startsection{subsection}{2}{0pt}%
    {-4pt plus -4pt minus -1pt}{2pt}{\AppendixFontSize\bf\RAGG}}
  \def\subsubsection{\@startsection{subsubsection}{3}{0pt}%
    {3pt plus 3pt minus 1pt}{-1em}{\AppendixFontSize\bf}}
  \if@MOOR
    \def\section{\@startsection{section}{1}{1em}{12pt plus 2pt minus 4pt}{-1em}{\bf}}%
    \def\subsection{\@startsection{subsection}{2}{1em}{12pt plus 2pt minus 2pt}{-1em}{\bf}}%
    \def\subsubsection{\@startsection{subsubsection}{3}{1em}{12pt plus 2pt minus 2pt}{-1em}{\bf}}%
  \fi
  \if@OPRE
    \def\section{\@startsection{section}{1}{0pt}%
      {-6pt plus -6pt minus -1pt}{2.5pt}{\AppendixSectionHeadSize\sffamily\bfseries\RAGG}}
    \def\subsection{\@startsection{subsection}{2}{0pt}%
      {-4pt plus -4pt minus -1pt}{2pt}{\AppendixFontSize\sffamily\bfseries\RAGG}}
    \def\subsubsection{\@startsection{subsubsection}{3}{0pt}%
      {3pt plus 3pt minus 1pt}{-1em}{\AppendixFontSize\bf}}
  \fi
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \setcounter{subsubsection}{0}%
  \renewcommand\thesection{\@Alph\c@section}%
  \parindent1em}
  {\vskip1sp}


\def\AppendixHeadSize{\fs.13.15.\relax}
\def\AppendixFontSize{\small}
\def\AppendixSectionHeadSize{\fs.11.{13.6}.\relax}

\if@MOOR
\let\AppendixHeadSize=\normalsize
\let\AppendixFontSize=\normalsize
\let\AppendixSectionHeadSize=\normalsize
\fi

\if@OPRE
\let\AppendixHeadSize=\normalsize
\let\AppendixFontSize=\normalsize
\let\AppendixSectionHeadSize=\normalsize
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%-e-Appendix

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ECSwitch{%
\clearpage
%\SingleSpaced
\normalsize
\pagestyle{ECheadings}%
\ECHowTheorems
\ECHowEquations
\ECHowSections
\setcounter{figure}{0}%
\renewcommand\thefigure{EC.\@arabic\c@figure}%
\setcounter{table}{0}%
\renewcommand\thetable{EC.\@arabic\c@table}%
\setcounter{page}{1}\def\thepage{ec\arabic{page}}%
\hspace*{1em}\relax}

\long\def\ECDisclaimer{\par\noindent{\fs.15.20.\raggedright\bf This page is intentionally blank.
Proper e-companion title page, with INFORMS branding and exact metadata
of the main paper, will be produced by the INFORMS office when the issue is being assembled.\endgraf}\clearpage}



\frenchspacing
\parindent 1em

\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% end of informs2.cls


